Enhancing Large Language Models for Hardware Verification: A Novel SystemVerilog Assertion Dataset

Hardware verification is crucial in modern SoC design, consuming around 70% of development time. SystemVerilog assertions ensure correct functionality. However, existing industrial practices rely on manual efforts for assertion generation, which becomes increasingly untenable as hardware systems become complex. Recent research shows that Large Language Models (LLMs) can automate this process. However, proprietary SOTA models like GPT-4o often generate inaccurate assertions and require expensive licenses, while smaller open-source LLMs need fine-tuning to manage HDL code complexities. To address these issues, we introduce **VERT**, an open-source dataset designed to enhance SystemVerilog assertion generation using LLMs. VERT enables researchers in academia and industry to fine-tune open-source models, outperforming larger proprietary ones in both accuracy and efficiency while ensuring data privacy through local fine-tuning and eliminating costly licenses. The dataset is curated by systematically augmenting variables from open-source HDL repositories to generate synthetic code snippets paired with corresponding assertions. Experimental results demonstrate that fine-tuned models like Deepseek Coder 6.7B and Llama 3.1 8B outperform GPT-4o, achieving up to 96.88% improvement over base models and 24.14% over GPT-4o on platforms including OpenTitan, CVA6, OpenPiton and Pulpissimo. VERT is available at https://github.com/AnandMenon12/VERT.

==> Algorithms/case_algo.tex <==

\begin{algorithm}[h]
\caption{Case Statements and Assertion Generation}
\label{alg:case}
\begin{algorithmic}[1]

\STATE \textbf{Input:} Input file $F_1$ (conditions), $F_2$ (variables)
\STATE Initialize an empty list $O$ for output

\STATE Load $F_1$ into datastructure $D_1$
\STATE Load $F_2$ into datastructure $D_2$

\STATE $S \gets \text{Select lines from } D_2$

\FOR{each $C_i \in S$}
    \STATE Initialize empty lists $A_i$ and $CS$
    
    \STATE $P \gets \text{Random unique conditions or variables from } D_1 or D_2 $

    \STATE Initialize arrays $PreCond$ and $PostCond$ of size len($P$) + 1
    \FOR{each row $i$ in $PreCond$ and $PostCond$}
        \STATE Fill $PreCond[i]$ with unique random elements from $D_2$
        \STATE Fill $PostCond[i]$ with unique random elements from $D_1$
    \ENDFOR
    
    
    \STATE $CS_i \gets \text{case ( } C_i \text{ )}$
    
    \FOR{each condition $p_j \in P$}
        \STATE Append condition $p_j$
        \STATE Append $PreCond[j] \text{ = } PostCond[j] $ to $CS_i$
    \ENDFOR
    
    \STATE Append default condition $PreCond$[len($P$) + 1]$\text{ = } PostCond$[len($P$) + 1]  to $CS_i$
    
    \STATE Initialize an empty string $A$ for assertions
    
    \FOR{each depth $d \in P$ + 1}
        \STATE Append property assertion based on $C_i$ and depth $d$ to $A$
    \ENDFOR
    
    \STATE Append final default assertion to $A$

    \STATE Append $CS_i$ and $A$  to $O$
    
\ENDFOR

\STATE \textbf{Output:} $O$

\end{algorithmic}
\end{algorithm}

The case dataset is essential for automating the verification of Verilog-style case statements, a critical step in hardware design verification. In complex digital systems, manually crafting exhaustive assertions for their respective case blocks can be error-prone and inefficient. An LLM fine-tuned on the case dataset can help automate comprehensive coverage of various case statements seen in Verilog code. Algorithm \ref{alg:case} showcases the generation of our synthetic case statements and their corresponding assertions. The algorithm operates by extracting select lines from a dataset of variables and conditions, and for each line, it constructs a Verilog-style case block. It randomly selects unique conditions and populates assignment operations. Since the conditional statements and assignment operation are known during the dataset generation process, the assertions can be constructed based on these conditions, ensuring consistency. The key steps of the algorithm are explained as follows:


In lines 1-2, the algorithm begins by accepting two input files: $F_1$, which contains the unique conditions, and $F_2$, which contains the variables. These two files provide the necessary data for constructing both the case statements and the assertions. An empty list $O$ is initialized to store the generated case statements and assertions. The input files $F_1$ and $F_2$ are then loaded into two separate data structures, $D_1$ and $D_2$, respectively, in lines 3-4. This enables efficient retrieval of relevant information from the datasets. Line 5 extracts the select lines/variables from $D_2$ and assigns them to the set $S$, which will be used to iterate over different cases. From line 6 onwards, for each select line $C_i$ in the set $S$, the algorithm initializes two empty lists: $A_i$ for storing assertions and $CS_i$ for holding the case statement being generated for the current select line. This process is outlined in line 7. Next, in line 8, a set of random unique conditions $P$ is selected from the datasets $D_1$ or $D_2$. These conditions determine the branching behavior within the case statement. In line 9, the algorithm initializes the arrays $PreCond$ and $PostCond$, which will store preconditions and postconditions for the case statement, respectively. The size of these arrays is determined by the length of the condition set $P$, incremented by one to accommodate a default condition. For each row, $i$ in $PreCond$ and $PostCond$ (lines 10-12), unique random elements are drawn from $D_2$ to fill $PreCond[i]$ and from $D_1$ to fill $PostCond[i]$. This ensures diversity in the conditions that the case statement will evaluate. 
Line 13 begins the construction of the case block by setting $CS_i$ as a Verilog-style case statement on the select line $C_i$. The algorithm then iterates through each condition $p_j \in P$ in lines 14-18. For each condition, the corresponding precondition $PreCond[j]$ and postcondition $PostCond[j]$ are appended to the case block, forming an assignment operation. In line 19, the default condition is appended to the case block. This condition uses the last elements of the precondition and postcondition arrays, ensuring that the case block handles scenarios where none of the predefined conditions are met. The default case is essential for comprehensive hardware design verification, as it ensures no undefined behavior occurs when the conditions in $P$ are not satisfied. Line 20 initializes an empty string $A$, holding the assertions to simulate formal verification. In lines 21-23, the algorithm iterates over each depth $d$ in $P$, generating property-based assertions for the current case. These assertions validate the logical flow between the select line $C_i$ and its associated conditions and paths. Each assertion ensures that if the select line $C_i$ matches a particular condition, the precondition leads to the expected postcondition, following property-based formal verification principles. In line 24, a final default assertion is appended to $A$, ensuring that even when the select line does not match any of the conditions in $P$, the default precondition and postcondition are correctly verified. This additional layer of verification ensures robustness in the hardware design. Finally, in line 25, the completed case statement $CS_i$ and its corresponding assertions $A$ are appended to the output list $O$. The process then repeats for each select line in $S$, generating new case statements and assertions until all cases have been processed. Once all cases are generated, the output list $O$ is returned in line 27, providing Verilog-style case statements and verification assertions.


%\as{Once you have the dataset, start talking about the LLM, what you plan to do with it..basically mention how other people can adapt your dataset to their model}

\subsubsection{Curated Dataset}

\begin{figure}
    \begin{subfigure}[c]{0.47\textwidth}
        %\hspace{-0.8cm}
        \input{Snippets/listing_ifelse}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[c]{0.06\textwidth}
        % \hspace{5mm}
        \includegraphics[width=\textwidth]{Figures/Chevron.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.47\textwidth}
        \input{Snippets/listing_ifelse_assertions}
    \end{subfigure}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%second row
    \begin{subfigure}[c]{0.47\textwidth}
        \input{Snippets/listing_case}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[c]{0.06\textwidth}
        % \hspace{5mm}
        \includegraphics[width=\textwidth]{Figures/Chevron.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.47\textwidth}
        \input{Snippets/listing_case_assertions}
    \end{subfigure}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%3 row
    \begin{subfigure}[c]{0.47\textwidth}
        \input{Snippets/listing_caseif}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[c]{0.06\textwidth}
        % \hspace{5mm}
        \includegraphics[width=\textwidth]{Figures/Chevron.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.47\textwidth}
        \input{Snippets/listing_caseif_assertions}
    \end{subfigure}
    \caption{Examples of code blocks (left) and their corresponding assertions (right) in our dataset.} % CLOCKWISE FROM TOP 
    \label{listings}
\end{figure}

We combine the \textbf{if else dataset} and \textbf{case dataset} to create a comprehensive dataset capable of addressing complex scenarios where ``if" and ``case" statements are nested within each other, accurately reflecting real-world programming and hardware description practices.


Figure \ref{listings} presents SystemVerilog code snippets and their formal assertions from our dataset. The left column shows representative code blocks with conditional and case-based logic. The top-left snippet is from the “if-else” dataset, where the assertion checks that when \texttt{!cfg\_7} is true and \texttt{hw\_13 \&\& reg\_14 || core\_17} holds, \texttt{chip\_9} must equal \texttt{fsm\_18}. This ensures correct signal assignment following the logic during simulation or formal verification.

The middle-left snippet, from the “case” dataset, assigns \texttt{chip\_12} to \texttt{tx\_10} if \texttt{flag\_register\_18} equals \texttt{5'b10011}. The corresponding assertion ensures that this assignment occurs correctly. The bottom-left snippet showcases a case statement where if \texttt{flag\_register\_18} is \texttt{7'h26} and the compound condition (\texttt{rx\_6 || rx\_1 || hw\_7}) holds, \texttt{cfg\_20} and \texttt{reg\_3} are assigned the expected values, formalized by an assertion.

Up to this point, the dataset has primarily focused on covering asynchronous cases, where the behavior of the hardware components and the conditions being tested do not rely on specific timing or clock cycles. These asynchronous scenarios are essential for verifying logic that operates independently of a clock signal. However, many real-world hardware systems depend heavily on synchronous behavior, driven by clock signals, to ensure proper timing and sequencing of operations. To address this, synchronous assertions are incorporated. These conditions utilize clock variables, such as\textit{ @(posedge clk\_i)}, extracted from open-source hardware projects. Including these clock-based conditions allows the dataset to accurately mimic the timing and synchronization behavior observed in actual hardware implementations, thus providing a robust tool for detailed verification and testing of hardware designs under various operational conditions. 

% Figure \ref{listings} presents a selection of SystemVerilog code snippets and their associated formal assertions drawn from our dataset. The left column contains representative code blocks involving conditional and case-based logic. The top-left code block showcases a snippet from the ``if-else" dataset. The first condition checks if the configuration signal \texttt{cfg\_7} is disabled (\texttt{!cfg\_7}). If this is true, the code triggers a sequence of operations. In the \texttt{else if} branch, another set of conditions is evaluated: if both \texttt{hw\_13} and \texttt{reg\_14} are true, or if \texttt{core\_17} is true, the signal \texttt{chip\_9} is assigned the value \texttt{fsm\_18}. The corresponding assertion ensures that the expected behavior occurs when these conditions are met. Specifically, it checks if \texttt{!cfg\_7} is true and if \texttt{hw\_13 \&\& reg\_14 || core\_17} holds. If both conditions are satisfied, the assertion guarantees that \texttt{chip\_9} must be equal to \texttt{fsm\_18}. This formalizes the behavior described in the code, ensuring that the signal assignment follows the conditional logic during simulation or formal verification.

% The middle-left code block features a snippet from the ``case" dataset that evaluates the value of \texttt{flag\_register\_18}. If \texttt{flag\_register\_18} equals the binary value \texttt{5'b10011}, the code assigns \texttt{chip\_12} to the signal \texttt{tx\_10}. The corresponding assertion formalizes this behavior. The property checks that if \texttt{flag\_register\_18} equals \texttt{5'b10011}, the signal \texttt{chip\_12} must indeed be assigned the value \texttt{tx\_10}. This ensures that the signal logic for \texttt{flag\_register\_18} is correctly implemented and verified, confirming that \texttt{chip\_12} will have the correct value under this specific case.

% The bottom-left block shoecases a datapoint from the case dataset with an if statement nested within. The case statement checks if \texttt{flag\_register\_18} is equal to the hexadecimal value \texttt{7'h26}. If true, it evaluates a compound condition (\texttt{rx\_6 || rx\_1 || hw\_7}). If any of these signals are high, it assigns \texttt{err\_20} to \texttt{cfg\_20} and \texttt{rst\_15} to \texttt{reg\_3}, indicating some kind of error or reset state. The corresponding assertion formalizes this logic. It checks if \texttt{flag\_register\_18} is \texttt{7'h26} and if the compound condition (\texttt{rx\_6 || rx\_1 || hw\_7}) holds. If both are true, it asserts that \texttt{cfg\_20} must equal \texttt{err\_20} and \texttt{reg\_3} must equal \texttt{rst\_15}. This ensures that the case-based control flow and the corresponding signal assignments behave as expected, thus preventing potential misbehavior in the design.

% Up to this point, the dataset has primarily focused on covering asynchronous cases, where the behavior of the hardware components and the conditions being tested do not rely on specific timing or clock cycles. These asynchronous scenarios are essential for verifying logic that operates independently of a clock signal. However, many real-world hardware systems depend heavily on synchronous behavior, driven by clock signals to ensure proper timing and sequencing of operations. To address this, synchronous assertions are incorporated. These conditions utilize clock variables, such as\textit{ @(posedge clk\_i)}, extracted from open-source hardware projects. The inclusion of these clock-based conditions allows the dataset to accurately mimic the timing and synchronization behavior observed in actual hardware implementations, thus providing a robust tool for detailed verification and testing of hardware designs under various operational conditions. 


% Code block how 2 explain?

% TABLE TALKINGABOUT if-!case, case-!if, etc

% The algorithm takes an input file, as shown in line 1,  representing the input file of case variables.

% In line 2, an empty list $O$ is initialized, which will store the final output. The next steps (lines 3 and 4) involve loading the case variables from $F1$ into a data structure $D$. Following this, in line 5, an array of select line variables, denoted as $S$, is extracted from $D$.

% The main logic starts in line 6 with a loop iterating over each select line $C_i \in S$, where $C_i$ is the case name. For each case, empty lists $A_i$ (to store assertions) and $E_i$ (for explanations) are initialized (line 7). Line 8 generates a random integer $r$, representing the number of unique paths and preconditions to be selected.

% In lines 9 and 10, a set of $r$ unique paths $P$ is randomly chosen from the path variables in $D_1$, and $r$ unique preconditions $R$ are randomly selected from the precondition variables in $D_1$. The algorithm then initializes two-dimensional lists $PreCond$ and $PostCond$, with 1 row and $r$ columns, to store the randomly selected preconditions and postconditions, as shown in line 11.

% The loop in lines 12 through 14 fills the $PreCond$ and $PostCond$ lists with the selected values. The preconditions in $R$ are assigned to $PreCond[i]$ (line 13), while random postconditions from $D_1$ are assigned to $PostCond[i]$ (line 14).

% In line 16, both the $PreCond$ and $PostCond$ lists are converted into arrays for uniformity in data handling. The case statement construction begins in line 16, where $CS_i$ is initialized with the format \texttt{case ( } $C_i$ \texttt{ )}, using $C_i$ as the case variable. In the loop between lines 17 and 19, each selected path $p_j \in P$ is appended to the case statement. For each path, a condition that compares the precondition $PreCond[0][j]$ with the postcondition $PostCond[0][j]$ is generated and added to $CS_i$ (line 19).

% To complete the case statement, a random precondition and postcondition not present in $PreCond$ or $PostCond$ are chosen for the default case (lines 21 and 22), and the corresponding condition is appended to $CS_i$ (line 23).

% Next, the assertions corresponding to the case statements are generated in line 24. An empty string $A$ is initialized to store these assertions. The loop in lines 25 through 27 creates an assertion for each path depth $d \in P$. For each depth, a property assertion based on the case variable $C_i$ and depth $d$ is appended to the string $A$ (line 26). Finally, a default assertion is appended after the last path depth is processed (line 28).


% The algorithm concludes in line 31 by writing the output list $O$ to a JSON file, thereby generating the final synthetic dataset containing the case statements and assertions.



% Algorithm \ref{alg:case} begins by initializing an empty list, which will hold the synthetic case statements and assertions. It then loads an input file containing relevant variable names, which provides the case names for subsequent processing. The algorithm initializes two empty lists for each case name: one to hold the case-specific assertions and another to store assertions.

% A random integer is generated to determine the number of paths for each case. The algorithm then extracts the unique conditions from the input file, selecting a random subset of these conditions based on the previously generated integer. Similarly, it chooses a set of random preconditions and postconditions from the input file. The preconditions form the left-hand side (LHS) or the assignee of the assignment statements in the synthetic dataset, while the postconditions form the right-hand side (RHS) or the assigned value. 

% Next, two 2D arrays are initialized to store the preconditions and postconditions corresponding to the generated conditions. The algorithm fills these arrays by mapping the randomly selected preconditions to their respective postconditions, which are also chosen at random from the input data. 

% The core of the algorithm is the generation of case statements. For each case name, the algorithm constructs a case statement by iterating over the selected paths. For each path, it appends the corresponding preconditions and postconditions to the case statement, ensuring that the logical relationships are maintained. Additionally, the algorithm generates a default case using randomly selected preconditions and postconditions not previously used, which ensures that the case statement covers all possible scenarios.

% In parallel with the generation of case statements, the algorithm constructs the corresponding assertions. For each path, an assertion is created for the precondition that leads to the mapped postcondition. Furthermore, the algorithm includes a default assertion to simulate the verification conditions not explicitly covered by the paths.

% Finally, the algorithm appends the generated case statement, assertions, and a synchronous flag to the output list. Once all case names have been processed, the output is written to a JSON file. This synthetic dataset, containing the case statements and their corresponding assertions, ensures that the relationships between the case conditions and their verification steps are well-defined and consistent, making it suitable for model training.



% Algorithm \ref{alg:case} systematically generates synthetic case statements and their corresponding assertions. The algorithm begins by initializing an empty list $\mathcal{O}$ to store the generated case statements and assertions. It then loads data from a CSV file, which contains variables used to populate the case statements, and a JSON file that stores a dataset of pre-existing conditions. Next, the algorithm extracts the relevant control variables from the CSV file into an array $\mathcal{S}$, which serves as the input for generating each case statement.

% For each control variable $\mathcal{C}$, the algorithm generates random unique paths and conditions. These paths are selected from a set of unique paths present in the CSV file, while the conditions are drawn from a set of predefined preconditions, ensuring randomness and diversity in the dataset. Two lists, $\mathcal{C}_{\text{pre}}$ and $\mathcal{C}_{\text{post}}$, are initialized to store the preconditions and postconditions, respectively. These lists are populated by sampling random values from the available preconditions in the CSV file.

% Once the conditions are established, the algorithm constructs the body of the case statement, beginning with the case header. For each randomly selected path, a corresponding precondition and postcondition pair is appended to the case statement, ensuring that the logic follows the intended conditional behavior. A default case is also generated, which assigns randomly selected values for the precondition and postcondition not used in the previous paths, ensuring the completeness of the case statement.

% The next step involves generating the relevant assertions. For each path, the algorithm constructs an assertion that specifies the condition under which the precondition must hold true in relation to the postcondition. This ensures that the assertion precisely reflects the behavior encoded within the case statement. Additionally, the final assertion checks the behavior when none of the paths match, and the default case is triggered, reinforcing the correctness of the case structure.

% Finally, each generated case statement and its corresponding assertion are appended to the output list $\mathcal{O}$ and written to a file in JSON format. If this is the first case statement generated, the algorithm prints the case and assertion for verification. By carefully controlling the conditions and paths used to construct each case, the algorithm ensures that the generated assertions are valid and complete for each corresponding case statement.


%Now give a line by line explanation of the algorithm in Latex code for a section in an academic paper. Write it as a paragraph. DO NOT MENTION PYTHONIC TERMS. The code is used to generate a synthetic dataset containing case statements (don't just refer to them as conditional) and the relevant assertions. The idea is that since we are generating the if statements we know the conditions for the assertions. It need to be in Latex Code

%Now generate a latex algortithm for this pseudocode. use symbols instead of specific terms and focus on improving its readability. use \STATE not \State





==> Algorithms/conditions.tex <==
\begin{algorithm}[t]
\caption{Unique Conditions Generation}\label{alg:unique_identifiers}
\begin{algorithmic}[1]

\STATE \textbf{Input:} $V_{list}$ , $N_{cond}$
\STATE \textbf{Output:} Condition set $C_S$

\STATE Define operator list $O_p$

\STATE \textbf{Function} GenerateCondition($V$)
\STATE \quad Select operator $op \in O_p$
\STATE \quad Return condition by joining $V$ using $op$

\STATE \textbf{Function} GenerateData($V_{list}$, $N_{cond}$)
\STATE \quad Initialize empty set $D$
\STATE \quad \textbf{for}{ $i \in 1$ to $N_{cond}$} \textbf{do}
    \STATE \quad \quad Select random unique variables $V$ from $V_{list}$
    
    \STATE \quad \quad Generate conditions using GenerateCondition($V$)
    \STATE \quad \quad Append conditions and variables to $D$
\STATE \quad \textbf{endfor}
\STATE \quad Return $D$

\STATE Generate $C_S = $ GenerateData($V_{list}$, $N_{cond}$)
\STATE Save $C_S$ to file
\STATE Return $O$

\end{algorithmic}
\end{algorithm}

The next step in our approach involves generating a comprehensive set of conditions based on the cleaned variable list. These conditions serve as the foundation for creating structured code blocks, along with their corresponding assertions. By dynamically generating these conditions, we can ensure that the model is exposed to a wide array of patterns, preventing it from overly relying on specific naming conventions or design features commonly encountered in SoC components. 

Algorithm \ref{alg:unique_identifiers} showcases the proposed condition generation. The input to the algorithm is a list of variables $V_{list}$ and the number of conditions $N_{cond}$ that need to be generated. The output is a set of conditions $C_S$ containing the unique conditions generated during execution. In line 1, the list of variables $V_{list}$ is provided as input, along with the number of conditions $N_{cond}$ that need to be generated. The result of the algorithm is the condition set $C_S$, defined as the output in line 2. In line 3, the algorithm defines a list of operators $O_p$. These operators, such as logical and comparison operators, will be joined with the variables in $V_{list}$ to form the conditions. Lines 4 - 6 define the \texttt{GenerateCondition} function. This function takes a set of variables $V$ as input and generates a condition by selecting an operator $op\in O_p$ (line 5). The selected operator is then used to join the variables in $V$, and the generated condition is returned (line 6). Lines 7 to 13 describe the \texttt{GenerateData} function, which takes as input the list of variables $V_{list}$ and the number of conditions to generate $N_{cond}$. In line 8, the function initializes an empty set $D$ to hold the generated conditions. The algorithm then enters a loop (lines 9–12), iterating $N_{cond}$ times to generate the required conditions. In each iteration (line 10), a random subset of unique variables $V$ is selected from the list $V_{list}$. The selected variables are passed to the \texttt{GenerateCondition} function to generate a condition (line 11). The generated condition, along with the selected variables, is appended to the set $D$ (line 12). This process repeats until the specified number of conditions, $N_{cond}$, is generated. In line 13, the \texttt{GenerateData} function returns the set of conditions $D$. In line 14, the \texttt{GenerateData} function is called with $V_{list}$ and $N_{cond}$ as arguments to generate the final condition set $C_S$. The condition set $C_S$ is then saved to a file in line 15, and the condition set is returned as the output in line 16.


==> Algorithms/if_else_algorithm.tex <==

% \begin{algorithm}[h]
% \caption{Generation of If Assertions}
% \label{alg:if-else}
% \begin{algorithmic}[1]
% \STATE Initialize $\mathcal{O} \gets \emptyset$ \COMMENT{Output set}
% \STATE $\mathcal{D}_{\text{input}} \gets \text{Load Input Data}$ \COMMENT{Data for condition generation}
% \FOR{$\ell \in \mathcal{D}_{\text{input}}$}
%     \STATE Initialize $\mathcal{C}, \mathcal{P}, \mathcal{A}, \mathcal{U} \gets \emptyset$ \COMMENT{Condition depths, preconditions, assertions, used conditions}
%     \STATE Sample $\eta, \kappa, \gamma \sim \text{Random Distributions}$ \COMMENT{Randomly sample key parameters}
%     \STATE Sample $\mathcal{D}_{\text{cond}} \sim \text{Unique Conditions from Input}$ \COMMENT{Sample unique conditions}
%     \STATE Sample $\mathcal{D}_{\text{pre}} \sim \text{Preconditions from Input}$ \COMMENT{Sample unique preconditions}
    
%     \STATE Define $\textsc{SelectCond}(\alpha)$:
%     \STATE \hspace{0.5cm} Sample condition $\zeta \in \mathcal{D}_{\text{cond}}$
%     \STATE \hspace{0.5cm} Ensure $\zeta \notin \mathcal{U}$, resample if necessary
%     \STATE \hspace{0.5cm} Append $\zeta$ to $\mathcal{C}$ and update $\mathcal{U} \gets \mathcal{U} \cup \{\zeta\}$
%     \STATE \hspace{0.5cm} Return condition $\zeta$
    
%     \STATE Define $\textsc{SelectPre}()$: Append precondition from $\mathcal{D}_{\text{pre}}$ to $\mathcal{P}$
%     \STATE Define $\textsc{SelectPost}()$: Append postcondition from $\mathcal{D}_{\text{pre}}$ to $\mathcal{A}$

%     \STATE Construct conditional structure $\mathcal{S}_{\text{if}} \gets \text{if} (\ell)$
%     \FOR{$i = 1$ to $\kappa$}
%         \STATE $\mathcal{S}_{\text{if}} \gets \mathcal{S}_{\text{if}} \cup \textsc{SelectPre} = \textsc{SelectPost}$ \COMMENT{Construct main condition body}
%     \ENDFOR

%     \FOR{$j = 1$ to $\eta$}
%         \STATE $\zeta_j \gets \textsc{SelectCond}(\text{False})$
%         \STATE $\mathcal{S}_{\text{if}} \gets \mathcal{S}_{\text{if}} \cup \text{if} (\zeta_j)$
%         \FOR{$k = 1$ to $\kappa$}
%             \STATE $\mathcal{S}_{\text{if}} \gets \mathcal{S}_{\text{if}} \cup \textsc{SelectPre} = \textsc{SelectPost}$
%         \ENDFOR
%         \FOR{$m = 1$ to $\gamma$}
%             \STATE $\zeta_{j,m} \gets \textsc{SelectCond}(\text{True})$
%             \STATE $\mathcal{S}_{\text{if}} \gets \mathcal{S}_{\text{if}} \cup \text{else if} (\zeta_{j,m})$
%             \FOR{$k = 1$ to $\kappa$}
%                 \STATE $\mathcal{S}_{\text{if}} \gets \mathcal{S}_{\text{if}} \cup \textsc{SelectPre} = \textsc{SelectPost}$
%             \ENDFOR
%         \ENDFOR
%     \ENDFOR

%     \STATE Construct assertion $\mathcal{S}_{\text{assert}} \gets \text{Assert} (\ell)$ based on condition depth $\eta$
%     \FOR{$n = 1$ to $\eta$}
%         \STATE $\mathcal{S}_{\text{assert}} \gets \mathcal{S}_{\text{assert}} \cup (\mathcal{C}_n \rightarrow \textsc{SelectPre} = \textsc{SelectPost})$
%     \ENDFOR

%     \STATE Append $\mathcal{S}_{\text{if}}$ and $\mathcal{S}_{\text{assert}}$ to $\mathcal{O}$
% \ENDFOR
% \STATE Save $\mathcal{O}$ to external file.
% \end{algorithmic}
% \end{algorithm}

% The algorithm outlined in Algorithm~\ref{alg:if-else} generates a synthetic dataset containing if-else statements and their corresponding assertions. Initially, an output set $\mathcal{O}$ is initialized to store the generated data. The algorithm begins by loading the input data, $\mathcal{D}_{\text{input}}$, which provides the parameters for generating conditions and assertions. For each element $\ell$ in the input, several lists are initialized to track the condition depths ($\mathcal{C}$), preconditions ($\mathcal{P}$), assertions ($\mathcal{A}$), and already used conditions ($\mathcal{U}$) to avoid duplicates. The algorithm proceeds by sampling key parameters such as the number of conditions ($\eta$), the number of preconditions and postconditions within each statement ($\kappa$), and the number of else-if branches ($\gamma$) from predefined random distributions. These parameters govern the structure and depth of the generated if-else statements.

% A unique set of conditions ($\mathcal{D}_{\text{cond}}$) and preconditions ($\mathcal{D}_{\text{pre}}$) is sampled from the input data. The function $\textsc{SelectCond}(\alpha)$ is defined to select a new condition $\zeta$ for the current depth of the if-else tree. If a condition is already used, it is resampled until a unique one is found, ensuring no condition is reused inappropriately. The selected condition is appended to $\mathcal{C}$, and $\mathcal{U}$ is updated accordingly. Similarly, the functions $\textsc{SelectPre}()$ and $\textsc{SelectPost}()$ are defined to randomly select preconditions and postconditions and append them to their respective lists. 

% The core of the algorithm constructs the if-else structure, beginning with an initial if statement for each element $\ell$. The algorithm appends $\kappa$ number of assignments within the if block, pairing each precondition with its corresponding postcondition. The nested structure is built by iterating through the sampled number of conditions ($\eta$), where a new if statement is introduced for each condition depth. For each nested if, the algorithm appends further assignments linking preconditions and postconditions. Additionally, $\gamma$ number of else-if branches are created, using new conditions and inserting appropriate preconditions and postconditions.

% Once the if-else structure is generated, the algorithm constructs the corresponding assertion $\mathcal{S}_{\text{assert}}$. Since the conditions and their relationships are known, the assertions are generated based on the condition depth. The assertion ensures that for each condition in $\mathcal{C}$, the preconditions correctly imply the expected postconditions. Each generated if-else structure, along with its associated assertions, is appended to the output set $\mathcal{O}$, which is ultimately saved as a synthetic dataset containing both the if-else statements and their respective assertions.

% \begin{algorithm}[h]
% \caption{Generation of If Assertions}\label{alg:if-else}
% \begin{algorithmic}[1]
%     \STATE Initialize list $\mathcal{O}$ for output data.
%     \STATE Load table $\mathcal{T}$ from the CSV file.
%     \STATE Extract array $\mathcal{L}$ from the 'MainCondlength' column in $\mathcal{T}$.
    
%     \FOR{each $L_i$ in $\mathcal{L}$}
%         \STATE Initialize empty lists $\mathcal{D}$, $\mathcal{P}_{\text{Pre}}$, $\mathcal{P}_{\text{Post}}$, $\mathcal{A}$, and $\mathcal{E}$.
%         \STATE Initialize empty set $\mathcal{U}$ for used conditions.

%         \STATE Generate random integer $r \in $ (number of unique conditions).
%         \STATE Generate random integer $v \in $ (number of assertions per condition).
%         \STATE Generate random integer $n \in $ (number of \textbf{else if} statements).

%         \STATE Select $r$ unique values for condition depths $\mathcal{D}$ from $\mathcal{T}$.

%         \STATE Define function $\textsc{GetCond}(b)$ that:
%             \IF{$\mathcal{C} \notin \mathcal{U}$}
%                 \STATE Add condition $\mathcal{C}$ to $\mathcal{U}$.
%             \ELSE
%                 \REPEAT
%                     \STATE Select a new $\mathcal{C}$ until not in $\mathcal{U}$.
%                 \UNTIL{condition is unique.}
%             \ENDIF
%             \STATE Append condition to $\mathcal{D}$.
%             \IF{$b = \text{true}$}
%                 \STATE Return negated $\mathcal{C}$.
%             \ELSE
%                 \STATE Return $\mathcal{C}$.
%             \ENDIF

%         \STATE Define function $\textsc{GetPre}$ that selects and returns a precondition from $\mathcal{T}$.
%         \STATE Define function $\textsc{GetPost}$ that selects and returns a postcondition from $\mathcal{T}$.

%         \STATE Create initial \textbf{if} block for condition $L_i$.
%         \FOR{each $v_j$ from 1 to $v$}
%             \STATE Add precondition and postcondition to the \textbf{if} block.
%         \ENDFOR

%         \FOR{each $d_k$ from 1 to $r$}
%             \STATE Add a nested \textbf{if} block with condition $\textsc{GetCond}()$.
%             \FOR{each $v_j$ from 1 to $v$}
%                 \STATE Add assertions to the nested \textbf{if} block.
%             \ENDFOR
%             \FOR{each $n_l$ from 1 to $n$}
%                 \STATE Add an \textbf{else if} block with condition $\textsc{GetCond}(\text{true})$.
%                 \FOR{each $v_j$ from 1 to $v$}
%                     \STATE Add assertions to the \textbf{else if} block.
%                 \ENDFOR
%             \ENDFOR
%         \ENDFOR

%         \STATE Add a final \textbf{else} block with additional assertions.

%         \STATE Generate assertions for all nested conditions.
%         \FOR{each depth $d_k$}
%             \STATE Create property assertions for depth $d_k$.
%         \ENDFOR

%         \STATE Add generated code and assertions to $\mathcal{A}$.
%     \ENDFOR

%     \STATE Append generated code and assertions to $\mathcal{O}$.
%     \STATE Write $\mathcal{O}$ to a file.
% \end{algorithmic}
% \end{algorithm}

% The algorithm shown in algorithm \ref{alg:if-else} presented is designed to generate a synthetic dataset containing if-else statements and corresponding assertions. It begins by initializing an empty list, denoted as $\mathcal{O}$, which will store the generated output. The algorithm then reads data from a CSV file into a table, $\mathcal{T}$, and extracts a specific column, referred to as 'MainCondlength', into an array, $\mathcal{L}$. For each value in $\mathcal{L}$, several lists are initialized to track the condition depths ($\mathcal{D}$), preconditions ($\mathcal{P}{\text{Pre}}$), postconditions ($\mathcal{P}{\text{Post}}$), and assertions ($\mathcal{A}$). A set $\mathcal{U}$ is also initialized to track conditions that have already been used, ensuring uniqueness in condition generation.

% Next, random integers are generated: $r$ determines the number of unique condition depths, $v$ determines how many assertions are associated with each condition, and $n$ specifies the number of else if statements. The algorithm then selects $r$ unique values from the table for the condition depths. To manage condition generation, the algorithm defines a helper function, \textsc{GetCond}, which either returns a new condition or a negated condition, ensuring no duplication by checking against the set $\mathcal{U}$. Additional functions, \textsc{GetPre} and \textsc{GetPost}, are defined to retrieve random preconditions and postconditions from the table.

% Once these functions are defined, the algorithm constructs the main if block for each value in $\mathcal{L}$. Within this block, assertions are added based on randomly selected preconditions and postconditions. The algorithm then generates nested if statements up to $r$ levels deep, each with associated conditions and assertions. For each depth level, the algorithm adds the corresponding else if blocks, also populated with assertions based on the conditions defined earlier. A final else block is appended, containing additional assertions.

% After constructing the if-else structure, the algorithm generates assertions that correspond to the conditions in each depth level. These assertions are based on the preconditions and postconditions stored earlier, ensuring that the generated assertions align with the previously constructed conditions. The final code and assertions are appended to the list $\mathcal{O}$. Once the process completes, the algorithm writes the contents of $\mathcal{O}$ to a file in the desired format. This synthetic dataset provides a rich set of if-else statements, where the conditions for each assertion are known, enabling the dataset to be used for validation purposes or further study of logical inference and condition handling.


\begin{algorithm}[h]
\caption{Generation of If-else Assertions}\label{alg:if-else}
\begin{algorithmic}[1]

\STATE \textbf{Input:} Input file $F_1$ (conditions), $F_2$ (variables)
\STATE Initialize an empty list $O$ for output
\STATE Load $F_1$ into datastructure $D_1$
\STATE Load $F_2$ into datastructure $D_2$
\STATE $S \gets$ Select unique conditions from $D_1$
\FOR{each $C_i \in S$}
    \STATE Initialize empty lists $A_i$ and $IS_i$
    \STATE Initialize $PreCond$ and $PostCond$ of size $N$
    \STATE Fill $PreCond$ with unique random elements from $D_2$
    \STATE Fill $PostCond$ with unique random elements from $D_1$ or $D_2$
    \STATE $IS_i \gets if ( C_i ) $
        \STATE Append $PreCond$[0] = $PostCond$[0] to $IS_i$

    \FOR{$i \in 1$ to $N$ - 1}
        \STATE Append else-if conditions to $IS_i$
        \STATE Append $PreCond$[i] = $PostCond$ to $IS_i$[i]
    \ENDFOR
    \STATE Append else statement to $IS_i$
    \STATE Append  $PreCond$[$N$] = $PostCond$[$N$] to $IS_i$
    \STATE Initialize an empty string $A$ for assertions
    \FOR{each depth $d \in N$}
        \STATE Append property assertions for $C_i$ and depth $d$ to $A$
    \ENDFOR
    \STATE Append final else assertion to $A$
    \STATE Append $IS_i$ and $A$ to $O$
\ENDFOR

\STATE \textbf{Output:} $O$

\end{algorithmic}
\end{algorithm}
%\as{why is if dataset part needed? small overview, }


The \textit{if-else} dataset is crucial for generating a diverse set of \textit{if-else} conditions that can be used to test and validate the behavior of systems under different logical scenarios. By automating the creation of conditional statements and their corresponding assertions, this dataset provides a structured approach for evaluating how systems handle various decision paths, making it an invaluable resource for hardware verification. Algorithm \ref{alg:if-else} shows how we construct a dataset of \textit{if-else} code blocks and their corresponding assertions by iterating over a set of conditions extracted from the previously generated dataset. The key steps of the algorithm are explained as follows:


In line 1, the algorithm takes two input files: $F_1$, which contains condition variables, and $F_2$, which contains the variables used to generate preconditions and postconditions. Here, preconditions refer to the left-hand side (LHS) or the assignee in an assignment statement, while postconditions refer to the right-hand side (RHS) or the assigned value. The output $O$ is initialized as an empty list (line 2) to store the generated code and assertions. In lines 3 and 4, the files $F_1$ and $F_2$ are loaded into respective data structures $D_1$ and $D_2$, where $D_1$ holds the condition data and $D_2$ holds the general variable data. Line 5 selects conditions $S$ from the data structure $D_1$. These lines contain the main conditions that will be used in the \textit{if-else} generation process. For each condition $C_i \in S$ (line 6), the algorithm initializes two empty lists, $A_i$ and $IS_i$ (line 7), to store the assertions and the \textit{if-else} block being generated. Line 8 initializes and fills the $PreCond$ and $PostCond$ lists, which store the preconditions and postconditions used within the \textit{if} and \textit{else-if} statements. Each list of size $N$ represents the depth of the \textit{if-else} code block and, subsequently, the number of assertions. It is important to note that we generate one assertion to represent each level in the \textit{if-else} code block. Here, $PreCond$ is filled with unique random elements from the variable dataset $D_2$ as the assignee is often a unique variable being assigned a value. Meanwhile, $PostCond$ is filled with random elements from either condition data structure $D_1$  or the variable data structure $D_2$. This is done as the assigned values could be variables or conditions themselves. In lines 11 and 12, the \textit{if} statement $IS_i$ is initialized, where the condition $C_i$ is used as the primary condition. This is the starting point for generating the nested \textit{if-else} block. The algorithm then appends the first statement in the form $PreCond[0] = PostCond[0]$ to the \textit{if} block. This defines the behavior of the system under the condition $C_i$. The nested structure is further expanded in lines 13-16, where a series of \textit{else-if} conditions are appended to $IS_i$ based on the depth $N$. In lines 17 - 18, the else statement is generated, and the final precondition and postcondition are selected for the else statement to simulate cases where none of the previous conditions hold. Line 19 initializes an empty string $A$ to store the assertions. Assertions are generated for each depth $d \in N$ (lines 20-22), simulating the validation of the \textit{if-else} structure at each level of nesting. Furthermore, these assertions correlate the same preconditions and postconditions to the specific level in the \textit{if-else} structure the assertion is meant to validate. Finally, in lines 23-24, the complete \textit{if-else} statement $IS_i$ and its corresponding assertions $A$ are appended to the output list $O$. This output contains the full generated structure, including the conditional logic and the assertions.

% \as{This gives the first component for our dataset- the if-else part}
% \as{can give an example of the generated assertion and corresponding code: for both case and if}

% \am{see \ref{listings}}



%The algorithm systematically constructs "if-else" blocks by selecting conditions from an input dataset, then procedurally adds assignment operations and assertions to simulate the validation of each conditional path.

==> Backup/Meth.tex <==
\section{Proposed \dataset framework generation}


\begin{figure}[t]
\centering
\includegraphics[width = \linewidth] {Figures/ICLR_2025.pdf}
\caption{Overview of our methodology.}
\vspace{-4mm}
  \label{fig:probstat}
\end{figure}


In this section, we provide a comprehensive overview of our proposed VERT framework for building the SystemVerilog assertion dataset. Figure \ref{fig:probstat} presents the process, which begins with collecting and cleaning data from open-source HDL projects, followed by generating relevant conditions and structuring the dataset. The next step involves fine-tuning LLMs using this dataset to train them in generating SystemVerilog assertions. Finally, we evaluate the fine-tuned models by testing them on industrial-grade SoCs to assess their effectiveness in producing valid and useful assertions for hardware verification. The following sections will explain each of these steps in detail.


\subsection{Data Collection and Cleaning}

Our approach begins by generating a comprehensive list of variable names for our dataset. To achieve this, we use variables extracted from hardware modules in open-source  Hardware description languages (HDL)  projects. HDLs like SystemVerilog rely heavily on variables to represent essential hardware design elements. By drawing from a diverse range of open-source modules, we ensure the model is exposed to various real-world scenarios. However, many SoC designs often reuse IP blocks from the same vendors, leading to variable names overlapping. Furthermore, similar IPs—such as different implementations of AES encryption—frequently perform the same operations, further contributing to the similarity in variable naming. This reuse and overlap, common in open-source and commercial SoCs, can introduce a degree of homogeneity in the design landscape. As a result, we introduce randomly generated variables to break this pattern and prevent the model from overfitting to specific naming conventions or operations commonly found in these IP blocks. Once the variable list is compiled, it undergoes a thorough cleaning process, which includes removing duplicates, resolving inconsistencies, and verifying syntactic correctness.




% The inclusion of randomly generated variables is key to reducing model bias and ensuring a balanced representation, reducing the risk of overfitting to specific patterns or naming conventions. Extracting variable names from real-world HDL projects further enriches the list by incorporating practical use cases.

\subsection{Condition Generation}

\input{Algorithms/conditions}


\subsection{Dataset Generation}

The dataset generated in this work consists of Verilog-style code blocks, specifically focusing on \textit{if-else} and \textit{case} statements alongside their corresponding verification assertions. Each code block is designed to simulate conditional hardware logic. The dataset encapsulates multiple scenarios, ensuring a wide range of logical conditions are covered. In addition to the code blocks, formal verification assertions are generated for each path within the conditional statements. This combination of code and verification assertions provides a comprehensive framework for automated hardware design verification, simulating both specific cases and default conditions. Further subsections will explore the structure of the \textit{if-else} and \textit{case} statements datasets in greater detail, highlighting the generation process and the logic underlying each verification assertion.

\subsubsection{IF-ELSE dataset Generation}
\input{Algorithms/if_else_algorithm}
\subsubsection{Case dataset Generation}
\input{Algorithms/case_algo}




%The process begins by adapting the raw dataset into a format that aligns with the input structure expected by the pre-trained model. This involves creating prompt templates that incorporate previously generated HDL code and the relevant assertions into the LLM system prompt. Following this, the LoRA (Low-Rank Adaptation) technique is applied to efficiently fine-tune the model by modifying only a subset of model parameters. Concurrently, a specific set of hyperparameters is carefully selected and adjusted, as outlined in Table~\ref{tab:param}, to optimize the fine-tuning process. These hyperparameters are tested to ensure they yield the best results for generating assertions tailored to hardware verification across multiple SoCs, detailed in Section~\ref{sec:results}. An explaination of the selected hyperparameters follows:


% We employed the Low-Rank Adaptation (LoRA) technique to enhance the model's ability to adapt to hardware verification tasks without extensively retraining the underlying neural network. Specifically, we utilized a LoRA rank of 256, which we determined provided an optimal balance between the model’s capacity for task-specific adaptation and the computational demands imposed by higher ranks. Additionally, we configured the LoRA alpha parameter to match the LoRA rank, setting both to 256. This configuration was chosen to maintain a scaling factor of 1, ensuring that the low-rank updates were adequately scaled to preserve the original model dynamics while introducing necessary task-specific modifications.

% We used a maximum sequence length of 4096 tokens, which is essential for processing longer input sequences in assertion generation, where extensive logic and condition sequences must be handled without truncation. We limited the number of training epochs to 3, as further training tended to increase overfitting on our dataset, thereby inhibiting the model’s ability to generalize effectively to unseen data, consequently diminishing its overall performance and robustness. A batch size of 64 was chosen to balance computational resource availability with the stability of convergence. The learning rate was set to $1.00e^{-04}$, identified as optimal during our experimentation, allowing the model to converge at a reasonable pace without overshooting the optimal point in the loss landscape. Finally, training was performed using Bf16 precision, which speeds up the training process while maintaining adequate stability.

% Furthermore, we specifically target certain layers of the LLMs to enhance adaptation quality while managing computational costs. The \texttt{Query}, \texttt{Key}, \texttt{Value}, \texttt{Output}, and \texttt{Gate} layers were selected for training. This approach ensured that merely 4-6\% of the model's parameters required training, while still preserving a high level of adaptation quality.

% \as{give paragraph, explain the hyperparamter table through a paragraph or two}

% \textbf{LoRA Rank}: We used Low-Rank Adaptation (LoRA) with a rank of 256. A rank of 256 provided sufficient capacity for our task while maintaining manageable computational demands.

% \textbf{LoRA Alpha}: The LoRA alpha parameter controls the scaling of the low-rank updates. Setting it to same value as the rank (256) ensured a scaling factor of 1, which allowed the updates to be adequately scaled.

% \textbf{Maximum Sequence Length}: A maximum sequence length of 4096 tokens was used to ensure that the model could process longer input sequences, which is particularly important in assertion generation tasks where sequences of conditions and logic must be handled without truncation.

% \textbf{Epochs}: We limited training to 3 epochs as we found that further training increased overfitting on the dataset, preventing the models from generalizing effectively to unseen data, thus reducing their overall performance and robustness.

% \textbf{Batch Size}: A batch size of 64 was selected as it offered a balance between computational resource availability and convergence stability.

% \textbf{Learning Rate}: A learning rate of 1.00E-04 was determined to be optimal during experimentation, as it allowed the model to converge at a reasonable pace without overshooting the optimal point in the loss landscape. 

% \textbf{Training Precision}: We used Bf16 (Brain Floating Point 16) precision. Bf16 allows us to speed up the training process while maintaining adequate stability.





%This methodology offers a scalable and efficient approach to automating hardware assertion generation. By leveraging advanced LLMs and real-world hardware platforms such as OpenTitan, OpenRISC, and CVA6, our approach streamlines the traditionally labor-intensive process of hardware verification. ction, designed to facilitate language model understanding.

% The algorithm outlined in Algorithm~\ref{alg:if-else} generates a synthetic dataset containing if-else statements and their corresponding assertions. Initially, an output set $\mathcal{O}$ is initialized to store the generated data. The algorithm begins by loading the input data, $\mathcal{D}_{\text{input}}$, which provides the parameters for generating conditions and assertions. For each element $\ell$ in the input, several lists are initialized to track the condition depths ($\mathcal{C}$), preconditions ($\mathcal{P}$), assertions ($\mathcal{A}$), and already used conditions ($\mathcal{U}$) to avoid duplicates. The algorithm proceeds by sampling key parameters such as the number of conditions ($\eta$), the number of preconditions and postconditions within each statement ($\kappa$), and the number of else-if branches ($\gamma$) from predefined random distributions. These parameters govern the structure and depth of the generated if-else statements.

% A unique set of conditions ($\mathcal{D}_{\text{cond}}$) and preconditions ($\mathcal{D}_{\text{pre}}$) is sampled from the input data. The function $\textsc{SelectCond}(\alpha)$ is defined to select a new condition $\zeta$ for the current depth of the if-else tree. If a condition is already used, it is resampled until a unique one is found, ensuring no condition is reused inappropriately. The selected condition is appended to $\mathcal{C}$, and $\mathcal{U}$ is updated accordingly. Similarly, the functions $\textsc{SelectPre}()$ and $\textsc{SelectPost}()$ are defined to randomly select preconditions and postconditions and append them to their respective lists. 

% The core of the algorithm constructs the if-else structure, beginning with an initial if statement for each element $\ell$. The algorithm appends $\kappa$ number of assignments within the if block, pairing each precondition with its corresponding postcondition. The nested structure is built by iterating through the sampled number of conditions ($\eta$), where a new if statement is introduced for each condition depth. For each nested if, the algorithm appends further assignments linking preconditions and postconditions. Additionally, $\gamma$ number of else-if branches are created, using new conditions and inserting appropriate preconditions and postconditions.

% Once the if-else structure is generated, the algorithm constructs the corresponding assertion $\mathcal{S}_{\text{assert}}$. Since the conditions and their relationships are known, the assertions are generated based on the condition depth. The assertion ensures that for each condition in $\mathcal{C}$, the preconditions correctly imply the expected postconditions. Each generated if-else structure, along with its associated assertions, is appended to the output set $\mathcal{O}$, which is ultimately saved as a synthetic dataset containing both the if-else statements and their respective assertions.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%CASE


% The algorithm presented in Algorithm \ref{alg:case} systematically generates a synthetic dataset consisting of case-based conditional structures and corresponding assertions. It begins by initializing an empty output set $\mathcal{O}$ and loading the input data $\mathcal{D}{\text{input}}$, which contains the variables necessary for generating case statements. For each case variable $c$ in the dataset, the algorithm samples key parameters, including $\eta$, the number of unique paths, and preconditions $\mathcal{D}{\text{pre}}$ from the input data. The selected paths $\mathcal{L}{\text{path}}$ and preconditions are then organized into two-dimensional structures $\mathcal{M}{\text{Pre}}$ and $\mathcal{M}_{\text{Post}}$, mapping preconditions to their corresponding postconditions.

% Next, the algorithm constructs a case statement, $\mathcal{S}{\text{case}}$, with each unique path condition from $\mathcal{L}{\text{path}}$ appended alongside its respective preconditions and postconditions. A default case is also generated, where both preconditions and postconditions are sampled from unused values to ensure diversity within the dataset. After constructing the case structure, the algorithm proceeds to generate assertions. For each depth within the path set, a corresponding assertion is created by comparing preconditions to postconditions, thus embedding logical correctness within the synthetic case statement. Additionally, a final assertion is constructed for the default case, ensuring that if none of the paths are matched, the default condition is asserted.

% The case statement and its corresponding assertions are then appended to the output set $\mathcal{O}$, which continues to accumulate similar synthetic cases. Finally, the output set $\mathcal{O}$ is saved as a synthetic dataset for subsequent analysis, ensuring that each case structure is associated with its respective assertions, contributing to a comprehensive and logically consistent dataset.


%Now give a line by line explanation of the algorithm in Latex code for a section in an academic paper. Write it as a paragraph. DO NOT MENTION PYTHONIC TERMS. The code is used to generate a synthetic dataset containing case statements (don't just refer to them as conditional) and the relevant assertions. The idea is that since we are generating the if statements we know the conditions for the assertions. It need to be in Latex Code

%For example, consider a fragment of a SystemVerilog file from the OpenTitan repository:
% \begin{verbatim}
% module aes_core (
%     input  logic [31:0]  data_in,
%     output logic [31:0]  data_out,
%     input  logic         clk,
%     input  logic         reset_n
% );
% \end{verbatim}

% From this code snippet, our tool extracts the variable names:
% \begin{itemize}
%     \item \texttt{data\_in}
%     \item \texttt{data\_out}
%     \item \texttt{clk}
%     \item \texttt{reset\_n}
% \end{itemize}


% After cleaning the data, we proceed to generate a set of conditions. In this step, we select \textit{unique variable names} from the cleaned data and pair them with randomly assigned \textit{conditional operations}. These operations include traditional hardware constructs such as \textit{if-else} blocks, \textit{case statements}, and \textit{ternary expressions}. 

% Next, the generated variables and operations are combined to form complete conditions. For example, a condition could represent a hardware behavior where a signal is asserted based on the state of multiple control signals. The generated dataset also contains both \textit{synchronous} and \textit{asynchronous conditions}, which are crucial for accurtely reflecting the different operational modes present in modern hardware designs.

==> Backup/Results.tex <==
\section{Results}
\label{sec:results}



We evaluate \dataset through a two-phase methodology. In the first phase, we fine-tune our models and assess the syntactical correctness of the assertions generated by these models. In the second phase, we evaluate whether the generated assertions accurately describe the design's functionality and the coverage they achieve. The accuracy of representing the functionalities is tested using mutation testing, which is further elaborated in Section~\ref{sec:metrics}. For coverage analysis, we employ Complete Path Coverage (CPC) as the metric, ensuring all independent paths in the design automaton are traversed~\cite{tong2010defining}. Formal verification tools such as \cite{jasper} and simulation tools like \cite{vivado} are utilized throughout both phases to validate correctness, representational accuracy, and achieving up to 100\% coverage.


\subsection{Experimental Setup}

In our experiments, we employed two prominent open-source large language models—LLama 3.1 8B and DeepSeek Coder 6.7B—to assess code generation for hardware design verification tasks. {\color{blue}LLama 3.1 8B was chosen for its efficiency and robust performance across various natural language processing tasks, offering rapid inference and resource efficiency that facilitate swift experimental iterations. In contrast, DeepSeek Coder 6.7B has been specifically fine-tuned for code generation, demonstrating a strong aptitude for producing syntactically correct and functionally relevant code.} By leveraging these two models, we aim to benchmark the effectiveness of our dataset, \dataset, across both general-purpose and code-specialized architectures, thereby providing a balanced assessment of diverse fine-tuning strategies.

Furthermore, since we cannot fine-tune GPT-4o due to it being a proprietary model, we compare the open-source fine-tuned models to GPT-4o to highlight the effectiveness of \dataset. To assess their ability to generate code across diverse coding conventions and design principles, we test them on three open-source SoC designs—OpenTitan \cite{opentitan_2024}, CVA6 \cite{zaruba2019cost}, and Pulpissimo \cite{8640145}. Our experimental platform comprises an Nvidia DGX server equipped with four Nvidia A-100 80GB GPUs.


\subsection{Evaluation Metrics} 
\label{sec:metrics}
The evaluation focuses on three primary metrics: (1) the total number of generated assertions, (2) the percentage of syntactically correct assertions, and (3) the percentage of functionally correct assertions. Syntactic correctness refers to adherence to hardware description language standards, while functional correctness indicates that the assertions accurately reflect the intended hardware behavior. 



%Through this comprehensive evaluation, we ensure that the generated assertions not only meet syntactical and functional criteria but also enhance the quality of verification for hardware IPs.

% \subsection{Difference between functional and syntactical assertions}
\input{Appendix_syn_func/textbox}

 % In this section, we delve into the nuances that separate syntactical errors—such as incorrect use of operators—from functional errors that result in misrepresentation of design logic.
 
% write about syntactical correctness
% To ensure comprehensive validation, we employ a two-stage process. First, we use simulation in Xilinx Vivado~\cite{vivado} to verify assertions involving asynchronous resets, as formal verification tools such as Cadence JasperGold~\cite{jasper} assume that asynchronous reset signals remain inactive during execution~\cite{miftah2024system}. Second, we assess the functional correctness of the assertions through both formal and simulation verification runs, confirming that they can be triggered and observed during testing.  

% Since formal tools like \cite{jasper} assume that asynchronous reset signals remain inactive during execution \cite{miftah2024system}, we use simulation in \cite{vivado} to verify assertions involving asynchronous resets and ensure the asserted properties can be covered. Next, we validate the functional correctness of the assertions by performing formal and simulation verification runs, validating that the assertions can be triggered and observed during testing. This two-stage process ensures that only syntactically correct and functionally valid assertions are retained in the design. Textbox \ref{tb:diff_func_syn} illustrates the difference between syntactical and functional errors in assertions within a hardware design context. It presents two issues that can arise when writing assertions to verify system behavior.

% This rigorous approach guarantees that only syntactically correct and functionally valid assertions are integrated into the design. Textbox~\ref{tb:diff_func_syn} further illustrates the distinction between syntactical and functional errors in assertions within a hardware design context.


We evaluate the functional correctness of the generated assertions through a two-step process that combines mutation testing with formal and simulation-based verification. First, we introduce mutation testing—consistent with the methodology in \cite{iman2024artmine}—by intentionally inserting small, targeted code modifications (mutants) into the design. These mutants deviate from the expected assertion logic, serving as benchmarks to verify that the assertions are effective in detecting logical inconsistencies. If a mutant does not trigger the corresponding assertion, that assertion is deemed functionally incorrect.

Next, we employ Jasper Gold, a fast formal verification tool, to check whether the mutations trigger the assertions~\cite{jasper}. Jasper Gold’s speed and formal analysis capabilities allow us to efficiently identify any functional errors. However, formal tools like Jasper Gold assume that asynchronous reset signals remain inactive during execution \cite{miftah2024system}, which means they cannot verify properties that involve asynchronous resets.

To address this limitation, we simulate the mutated design using Xilinx Vivado~\cite{vivado}. This simulation step ensures that assertions involving asynchronous resets are adequately covered, thereby complementing the formal verification stage. By combining mutation testing with both formal verification via Jasper Gold and simulation via Vivado, we ensure that only syntactically correct and functionally valid assertions are retained in the design.

This comprehensive approach not only confirms the robustness and relevance of the generated assertions—demonstrated by their high mutation detection rates across various benchmarks—but also guarantees complete coverage of conditional branches and critical logic paths within the hardware design. Textbox~\ref{tb:diff_func_syn} further illustrates the distinction between syntactical and functional errors in assertions within a hardware design context.
 
 %Since formal tools like Cadence JasperGold~\cite{jasper} assume that asynchronous reset signals remain inactive during execution~\cite{miftah2024system}, we use simulation in Cadence Vivado~\cite{vivado} to verify assertions involving asynchronous resets and ensure the asserted properties can be covered. Next, we validate the functional correctness of the assertions by performing formal and simulation verification runs, validating that the assertions can be triggered and observed during testing. This two-stage process ensures that only syntactically correct and functionally valid assertions are retained in the design. Textbox \ref{tb:diff_func_syn} illustrates the difference between syntactical and functional errors in assertions within a hardware design context.
 

 It presents two issues that can arise when writing assertions to verify system behavior.

\paragraph{Design Source Code:}
The provided SystemVerilog code in Textbox\ref{tb:diff_func_syn} shows an \texttt{always\_ff} block, triggered by either the rising edge of \texttt{clk\_aon\_i} or the falling edge of \texttt{rst\_aon\_ni}. The block resets or updates the value of \texttt{wakeup\_timer\_cnt\_q} based on certain conditions:
\begin{enumerate}
    \item If \texttt{rst\_aon\_ni} is low (reset active), the counter is set to zero.
    \item If \texttt{wakeup\_timer\_cnt\_clr} or certain other signals are asserted, the counter is reset.
    \item Otherwise, the counter is updated with a new value from \texttt{wakeup\_timer\_cnt\_d}.
\end{enumerate}

\paragraph{Assertions:}
Two properties are presented, each demonstrating a different type of error:

\begin{itemize}
    \item \textbf{Syntactical Error:} \\
    In \texttt{property ResetTimer1}, the assertion attempts to check if the counter is reset when \texttt{rst\_aon\_ni} is low. However, it contains a \textbf{syntactical error}: instead of using the comparison operator \texttt{==} to check if \texttt{wakeup\_timer\_cnt\_q} equals zero, the assignment operator \texttt{=} is mistakenly used. This would result in a syntax error during compilation.
    
    \item \textbf{Functional Error:} \\
    In \texttt{property ResetTimer2}, while the syntax is correct, the assertion misses an essential condition. It checks whether the counter is reset when the clear signal or related signals are asserted. However, it fails to include the reset condition (i.e., \texttt{if (!rst\_aon\_ni)}), resulting in a \textbf{functional error} because the assertion does not fully capture the intended behavior of the design, specifically missing the \texttt{if} condition from the original source code.
\end{itemize}

\paragraph{Key Point:}
We highlight how both types of errors (syntactical and functional) can undermine the correctness of assertions, either by preventing successful compilation (in the case of syntax errors) or by failing to accurately verify the design's intended behavior (in the case of functional errors).


% \subsection{Mutation Testing}
% \label{mutation}

% The functional correctness of the generated assertions was evaluated using mutation testing, consistent with the methodology outlined in \cite{iman2024artmine}. This approach involved introducing intentional, small code modifications (mutants) that deviated from the expected assertion logic. By detecting these mutants, we demonstrated the effectiveness of the generated assertions in identifying logical inconsistencies and validating their utility. Unlike trivial or redundant assertions (e.g., ``assert True''), these assertions were intricately aligned with the critical components of the hardware design, ensuring their relevance and impact.

% Our findings revealed that the generated assertions achieved up to 100\% functional correctness or ability to detect mutations across various benchmarks, underscoring their robustness and effectiveness. The same mutation testing methodology from \cite{iman2024artmine} was also applied to verify the importance of the generated assertions, further affirming their significance. This comprehensive evaluation highlighted the non-redundant nature of the benchmarks and the potential of LLMs fine-tuned on VERT for hardware verification. Furthermore, the method ensured complete coverage of conditional branches and critical logic paths within the hardware design. The LLM-generated assertions were specifically crafted to validate every logical path, leaving no branch or condition unchecked, thereby reinforcing their role in achieving thorough hardware verification.







\subsection{Data Leakage Verification}

\input{Tables/LeakageTable}

%\textcolor{blue}{Experiments and writing in progress}. 

Data leakage is a critical concern as it can lead to overestimated performance and misleading evaluations of model generalization. Preventing leakage is essential to ensure that the experimental results faithfully represent real-world performance and that benchmark comparisons remain fair. To ensure that no inadvertent data leakage occurs between \dataset and the evaluation benchmarks, we adopt a data leakage detection method based on byte-level 13-gram overlap. This approach, similar to that employed during the development of GPT-3, operates directly on the raw byte representations of the text, thus avoiding potential inconsistencies introduced by tokenization or encoding differences~\cite{brown2020language}.

We represent the text as a sequence of bytes, as shown in Eqn.~\ref{eqn:byteseq}. 

\begin{equation}
    b = (b_1, b_2, \ldots, b_L)
    \label{eqn:byteseq}
\end{equation}

Where $L$ is the length of the byte sequence. We define the set of all contiguous 13-grams extracted from this sequence as 
\begin{equation}
    N(b) = \{ (b_i, b_{i+1}, \ldots, b_{i+12}) \mid 1 \leq i \leq L-12 \}.
    \label{eqn:13gramseq}
\end{equation}

Suppose that $N_1$ and $N_2$ are the sets of 13-grams obtained from two corpora (e.g., our dataset and a benchmark). The degree of overlap between these two sets is quantified using the Jaccard similarity coefficient~\cite{jaccard1908nouvelles}, defined as
\begin{equation}
    \text{Overlap}(N_1, N_2) = \frac{|N_1 \cap N_2|}{|N_1 \cup N_2|},
\end{equation}
where \(|N_1 \cap N_2|\) is the number of common 13-grams between the two datasets, and \(|N_1 \cup N_2|\) is the total number of unique 13-grams present in either dataset.

A high overlap score (closer to 1) indicates a significant reuse of byte-level sequences between the datasets, potentially flagging data leakage. \textbf{Conversely, a low overlap score (closer to 0) suggests that the datasets are largely distinct}, thus reducing concerns about leakage. 

The results of our data leakage evaluation are summarized in Table~\ref{tab:LeakageTable}. The table is structured with the first column listing the benchmark or hardware IP under investigation. The subsequent four columns report the computed overlap scores using the byte-level 13-gram approach applied to different components: the \textit{Code Overlap Score} quantifies the overlap in the code segments; the \textit{Assertions Overlap Score} captures the overlap in assertion texts; and the \textit{DeepSeek Coder Prompt Overlap Score} as well as the \textit{LLama 3.1 Prompt Overlap Score} reflect the overlap in the respective prompt texts generated by these systems.

Examining the results, we observe that all overlap scores are very low, typically on the order of \(10^{-4}\). For instance, the \emph{Code Overlap Scores} across various benchmarks range from 0.0001 to 0.0005, which suggests minimal commonality in the underlying code. The \emph{Assertions Overlap Score} is consistently 0.0000 for all entries, indicating no detectable overlap in the assertion-related texts. Similarly, the overlap scores for both the DeepSeek Coder and LLama 3.1 prompts remain comparably low, with only minor variations observed across different benchmarks. These uniformly low scores confirm that there is negligible reuse of content between our dataset (\dataset) and the benchmark sources, thereby reinforcing the integrity of our evaluation framework against data leakage.


\input{Tables/hyperparam}
\subsection{Fine-Tuning Hyperparameters}
\label{sec:fine_tune}
We utilized the hyperparameters detailed in Table \ref{tab:param}, leveraging the Low-Rank Adapter (LoRA) technique with a rank and alpha of 256 to optimize the model for hardware verification tasks with minimal computational overhead. This configuration allowed for efficient low-rank updates, preserving the core model's behavior while integrating task-specific adjustments. A maximum sequence length of 4096 tokens was employed to accommodate longer logic and condition sequences in assertion generation, with training constrained to 3 epochs to avoid overfitting.  We selected a batch size of 64 and a learning rate of $1.00e^{-04}$ for computational efficiency and stable convergence, with Bf16 precision enhancing training speed without compromising accuracy. By targeting the \texttt{Query}, \texttt{Key}, \texttt{Value}, \texttt{Output}, and \texttt{Gate} layers, we effectively adapted the model while updating only 4-6\% of its parameters, thus optimizing performance while controlling computational costs.


\subsection{Evaluation Results}

%\subsubsection{Performance Comparison: Fine-Tuned Model vs. Base Model}

\input{Tables/asserttable}

Table \ref{tab:asserttable} compares the performance of the base and fine-tuned versions of the Llama 3.1 and DeepSeek Coder models across various hardware IP benchmarks. The first column of the table lists the benchmark name, such as OpenTitan/AES, where the SoC name (OpenTitan) is followed by the specific IP name (AES). The subsequent columns display the number of assertions generated and the percentage of those assertions that are both syntactically and functionally correct for both base and fine-tuned models. The table is organized by model type, with performance metrics broken down for each hardware IP block. Both the Llama 3.1 and DeepSeek Coder models demonstrated significant improvements over the base models following fine-tuning, with some benchmarks showing drastic gains. For Llama 3.1, syntactic correctness saw a maximum improvement of up to 83.33\%. Similarly, the functional correctness showed a maximum increase of 93.55\%. The DeepSeek Coder model exhibited similarly substantial improvements. For instance, syntactic correctness improved as much as 93.75\% (from 6.25\% to 100\%), and functional correctness increased up to 96.88\% (from 0\% to 96.88\%). These results highlight the effectiveness of fine-tuning in improving the models' ability to generate accurate hardware assertions.

%\subsubsection{Performance Comparison: Fine-Tuned Model vs. GPT-4o}
\begin{figure}[h]
    \begin{subfigure}[c]{0.49\textwidth}
        \includegraphics[width = \linewidth] {Figures/GPT-4_comp_syn.pdf}
        \caption{Comparison of GPT-4o and Fine-tuned model in Syntactically correct assertions.}
        \label{fig:gpt4_comp_syn}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[c]{0.49\textwidth}
        \includegraphics[width=\textwidth]{Figures/GPT-4_comp.pdf}
        \caption{Comparison of GPT-4o and Fine-tuned model in Functionally correct assertions.}
        \label{fig:gpt4_comp_fun}
    \end{subfigure}
    \caption{ Comparison of GPT-4o and Fine-Tuned Model Performance.}
    \label{fig:gpt4_Comp}
\end{figure}

To illustrate \dataset's effectiveness, we compare fine-tuned versions of the DeepSeek Coder and Llama 3.1 model with GPT-4o.
 
Figure \ref{fig:gpt4_comp_syn} and Figure \ref{fig:gpt4_comp_fun} show the syntactic and functional correctness of assertions generated by GPT-4o and the Fine-Tuned Llama 3.1 and Deepseek Coder models across various hardware benchmarks. The X-axis represents the benchmark SoC with its corresponding IP, such as OpenTitan AES, OpenTitan I2C, OpenTitan LC CTRL, and CVA6/Frontend, where assertions are evaluated. The Y-axis displays the percentage of correct assertions, indicating how reliably each model generated the assertions for each benchmark. Figure \ref{fig:gpt4_comp_syn} shows that fine-tuned Llama 3.1 and fine-tuned Deepseek Coder models significantly outperform GPT-4o by up to 20.69\% in generating syntactically correct assertions. In Figure \ref{fig:gpt4_comp_fun}, both Llama 3.1 and Deepseek Coder again outperformed GPT-4o by as much as 24.14\% and 21.02\% respectively, with functionally correct assertion in modules such as CVA6/Decode\&Issue and Pulpissimo/Debug unit. These results emphasize that LLMs fine-tuned on \dataset enhance not only syntactic correctness but also the functional reliability of the generated hardware assertions.


%\subsection{Mutation Testing}

% The functional correctness of the generated assertions was evaluated using mutation testing, consistent with the methodology outlined in \cite{iman2024artmine}. This approach involved introducing intentional, small code modifications (mutants) that deviated from the expected assertion logic. By detecting these mutants, we demonstrated the effectiveness of the generated assertions in identifying logical inconsistencies and validating their utility. Unlike trivial or redundant assertions (e.g., ``assert True''), these assertions were intricately aligned with the critical components of the hardware design, ensuring their relevance and impact.

% Our findings revealed that the generated assertions achieved up to 100\% functional correctness or ability to detect mutations across various benchmarks, underscoring their robustness and effectiveness. The same mutation testing methodology from \cite{iman2024artmine} was also applied to verify the importance of the generated assertions, further affirming their significance. This comprehensive evaluation highlighted the non-redundant nature of the benchmarks and the potential of LLMs fine-tuned on VERT for hardware verification. Furthermore, the method ensured complete coverage of conditional branches and critical logic paths within the hardware design. The LLM-generated assertions were specifically crafted to validate every logical path, leaving no branch or condition unchecked, thereby reinforcing their role in achieving thorough hardware verification.


\subsection{Ablation Study with Uncleaned Variable Names}


\input{Tables/abl_table}
Tables~\ref{tab:abl_table_syntactic} and~\ref{tab:abl_table_functional} present an ablation study with uncleaned variable names to highlight the impact of cleaning variable names on both syntactical and functional correctness. Table~\ref{tab:abl_table_syntactic} reports the results for Syntactically Correct Assertions (\%), while Table~\ref{tab:abl_table_functional} shows the results for Functionally Correct Assertions (\%).

In each table, Column~3 corresponds to assertions generated by the base model. Column~4 presents assertions generated by a model fine-tuned on a dataset containing syntactically incorrect variables (e.g., special characters not allowed in HDL languages). Column~5 shows results from a model fine-tuned on a dataset with duplicate variables that may skew the model’s learning and introduce ambiguity, and Column~6 reports results from a model fine-tuned on a dataset with inconsistent variables (such as conflicting variable names). Finally, Column~7 in each table reports the results using the cleaned variables that we ultimately use to build VERT.


The results reveal a clear trend across both syntactically and functionally correct assertions: cleaning variable names leads to dramatic improvements in performance. For instance, in Table~\ref{tab:abl_table_syntactic}, the base model for Llama~3.1 achieves only 29.92\% syntactically correct assertions on average, and this performance does not improve when the model is fine-tuned on data containing syntactically incorrect variables (dropping slightly to 29.08\%). In contrast, when the model is trained on data with duplicate variables, the average correctness nearly doubles to 76.36\%. This improvement continues with inconsistent variables (89.55\%), and ultimately, the highest performance of 92.79\% is reached once the variables are cleaned. A similar pattern holds for DeepSeek Coder, where the average syntactic correctness increases from around 20.9\% (base or syntactically incorrect) to 79.08\% with duplicate variables, 94.00\% with inconsistent variables, and peaks at 96.84\% with cleaned variables.

Table~\ref{tab:abl_table_functional} shows identical trends for functionally correct assertions. Llama~3.1’s base performance is at 13.73\%, with negligible change when trained on syntactically incorrect variables (13.76\%). However, exposure to duplicate variables boosts the average to 75.47\%, while training on inconsistent variables increases it further to 88.22\%. Cleaning the variables finally results in a remarkable 92.36\% average, indicating that proper variable naming is crucial not just for syntactical correctness but also for ensuring functional correctness. DeepSeek Coder exhibits a comparable progression, improving from a base of 15.97\% to 96.47\% with cleaned variables.

Notably, certain benchmarks highlight these effects even more starkly. For example, Llama~3.1’s performance on the OpenTitan/ADC CTRL benchmark jumps from 17.46\% (base) to 100\% with cleaned variables, and similar improvements are observed across various IPs. These results confirm that uncleaned or inconsistent variable names severely hinder the model’s ability to generate correct assertions. In contrast, cleaning the variable names not only rectifies the syntactical issues but also enables the models to generate assertions that are functionally more accurate, thereby validating our approach outlined in Section~\ref{sec:DatasetComposition} in building VERT.



% The results demonstrate that ignoring syntactically incorrect variable names has the most detrimental impact, as fine-tuned LLMs produce erroneous assertions when given incorrect variable names, resulting in worse performance than even the base models.


%that failing to address syntactically incorrect variable names is most detrimental—fine-tuned LLMs generate syntactically incorrect assertions when fed erroneous variable names, leading to lower performance compared to even the base models.

% Subsequently, LLMs fine-tuned with the cleaned variable list (VERT) achieved improvements of up to 17.76\% in syntactical correctness and 17.39\% in functional correctness compared to LLMs fine-tuned on a dataset that preserved duplicate variable names. This improvement is attributed to eliminating duplicates within the same assertion, thereby reducing ambiguity and enhancing the fine-tuned LLMs' ability to generate accurate results. Finally, addressing inconsistent variable names resulted in the smallest observed change, with improvements of up to 3.24\% in syntactical correctness and 4.81\% in functional correctness compared to LLMs fine-tuned on a dataset that maintained inconsistent variable names. This modest change is likely due to the fact that such inconsistencies represent a relatively minor portion of the overall variable list compared to duplicates and syntactically incorrect variables.

% \subsection{Examples comparing Fine-tuned model to Base model}
% \label{fine_base_assert_examples}
% In this section, we present a comparative analysis of the assertions generated by the base model versus those produced by the model fine-tuned on \dataset. By examining real-world examples from section \ref{}, we highlight the improvements in both syntactical and functional aspects achieved through fine-tuning.


% \subsubsection{OpenTitan Assertion examples}

% \label{open_assert_examples}

% In the base-model generated assertions, the chain of events depends on the reset signal. However, the assertion disables the `\texttt{rst\_ni}' signal. Moreover, the generated checking statement does not reflect the correct chain of events. `\texttt{edn\_req\_hold\_q}' should be assigned the current value of `\texttt{edn\_req\_hold\_d}', not the value it had in the previous clock cycle.
% \input{Appendix_examples_OpenTitan/Code_for_DEEPSEEK}

% \input{Appendix_examples_OpenTitan/Deepseek_example_listing_ND}


% \input{Appendix_examples_OpenTitan/Deepseek_example_listing}

% When generated by the same model fine-tuned on \dataset, it generates the assertions with `\texttt{rst\_ni}' under consideration, and it gets the correct clock cycle.

% \input{Appendix_examples_OpenTitan/CODE_for_LLAMA3}
% \input{Appendix_examples_OpenTitan/LLama3_example_listing_ND}

% Here, the base-model generated assertion does not get the chain of events right. The if-else block describes that if there is a reset invoked, `\texttt{lc\_state\_valid\_q}' is assigned $0$. Otherwise, it should be assigned the current value of `\texttt{lc\_state\_valid\_d}.' However, the generated assertion asserts that if `\texttt{!rst\_ni}' is risen, 
% `\texttt{lc\_state\_valid\_q}' should be assigned $0$, and in the next clock cycle, it should be assigned `\texttt{lc\_state\_valid\_d}.' 

% \input{Appendix_examples_OpenTitan/LLama3_example_listing}

% \subsubsection{CVA6 assertion examples}
% \label{cva6_assert_examples}
% In this case, the base model generated an always block that does not assert anything.
% \input{Appendix_examples_CVA6/Code_for_DEEPSEEK}
% \input{Appendix_examples_CVA6/Deepseek_example_listing_ND}

% In this case, the base model generated an always block that does not assert anything.

% \input{Appendix_examples_CVA6/Deepseek_example_listing}
% \input{Appendix_examples_CVA6/CODE_for_LLAMA3}
% \input{Appendix_examples_CVA6/LLama3_example_listing_ND}

% In this case, while the base model generated a syntactically correct property, it mistook the check condition as an edge-triggered event instead of a level-triggered event. Furthermore, it also got the clock cycle wrong. Instead of defining the property for the current clock cycle, it used the next clock cycle.

% \input{Appendix_examples_CVA6/LLama3_example_listing}

% \subsubsection{Pulpissimo assertion examples}
% \label{pulp_assert_examples}
% Here, the base model only checks whether the value of `\texttt{rdata\_sel\_q}' is within the defined parameters but not the operations.
% \input{Appendix_examples_Pulpissimo/Code_for_DEEPSEEK}
% \input{Appendix_examples_Pulpissimo/Deepseek_example_listing_ND}

% \input{Appendix_examples_Pulpissimo/Deepseek_example_listing}

% \input{Appendix_examples_Pulpissimo/CODE_for_LLAMA3}
% \input{Appendix_examples_Pulpissimo/LLama3_example_listing_ND}

% Here, the assertions miss the correct clock cycle for the assertions. Furthermore, it missed the nested conditional blocks under `\texttt{HRESETn},' which should have put the nested condition in an ``\texttt{AND}'' relation with `\texttt{HRESETn}.'

% \input{Appendix_examples_Pulpissimo/LLama3_example_listing}



\subsection{Examples of LLMs Fine-tuned on VERT Addressing GPT-4o Issues and Comparison With Human Experts}
In this section, we show how the intuition in dataset formulation, as discussed in Section 4.1 of our paper, translates into the effectiveness of the assertions generated by LLMs fine-tuned on VERT. Furthermore, we provide a comparison of these models with human experts. These scenarios include (1) clock cycle and pre-condition capturing, (2) relation representation for nested conditional blocks, and (3) handling long conditions. Each section begins with the relevant code snippet, followed by the assertions generated by each approach.


\subsubsection{ LLMs Fine-tuned on VERT vs. GPT-4o:\newline} 
\label{vertvsgpt4}

\textbf{Clock Cycle Misinterpretations:} We observe that LLMs often get confused between using the overlapping implication symbol ($|->$) and the non-overlapping symbol ($|=>$). To resolve clock cycle misinterpretation by LLMs, we standardized our format by using the overlapping implication symbol with a specified delay count and replacing the non-overlapping symbol. As shown in text box \ref{tbox:sv_clkcycle_appn} below, GPT-4o incorrectly uses the non-overlapping symbol, but both LLMs fine-tuned on VERT address this issue by correctly interpreting the clock cycle by using the overlapping implication symbol.
\input{Appendix_exmaples_Addressing_Issues/Clock_cycle}


\textbf{Miscapturing if Condition for else Branches:} LLMs often overlook the previous if/else if conditions when generating assertions for the subsequent else or else if branches in conditional statements. VERT addresses the common omission of conditions in the else/else-if branches of if-else statements by exposing the model to diverse conditional structures. As shown in text box \ref{tbox:sv_nestedIF_appn} below,  GPT-4o, in its second assertion, misses that the second assertion should verify that $monitor\_enable$ is \textit{FALSE} and $monitor\_enable\_q$ is \textit{TRUE}. However, both LLMs fine-tuned on VERT correctly identify these conditions and include them in the fourth generated assertion.


\textbf{Nested If-Else Conditions:} LLMs often struggle with generating assertions for deeply nested if-else conditions (i.e., blocks nested beyond two levels), which are common in hardware design. To address the challenge of LLMs struggling with deeply nested if-else statements, we expanded VERT to include complex, multi-level conditional structures. As illustrated by text box \ref{tbox:sv_nestedIF_appn} below, GPT-4o incorrectly represents the logic of a nested block. Specifically, it ignores the if condition and creates an assertion using a ternary operator, where the inner if condition is used as the test, the assignment is the \textit{TRUE} branch, and \textit{1'b1} is the \textit{TRUE} branch. However, both LLMs fine-tuned on VERT to correctly identify the correct nested statement and their conditions.

\textbf{Handling Long Conditions:} To address the challenge of generating accurate assertions for long and complex conditions, we expanded VERT to include a variety of cases where multiple conditions and operators must be evaluated simultaneously. As shown in textbox \ref{tbox:sv_long_appn} below, the source code requires any one of six conditions to be met before raising the $mr\_err$ flag. However, the generated output by GPT-4o creates three assertions for one flag change, each neglecting the other three conditions. This not only leads to incorrect assertions but also causes overhead in the number of assertions. However, both LLMs fine-tuned on VERT correctly generate a singular assertion that describes all the conditions and their relationships within the if-statement.

\input{Appendix_exmaples_Addressing_Issues/nested_if}





\input{Appendix_exmaples_Addressing_Issues/Long_Conditions}






\subsubsection{ LLMs Fine-tuned on VERT vs. Human Expert:\newline} 


Human experts and LLMs fine-tuned on \dataset generate assertions differently. Experts often create simpler, more readable assertions, reflecting a preference for human-friendly formats. LLMs, on the other hand, produce more standardized logical expressions. This difference highlights style preferences rather than superiority. Notably, despite these stylistic differences, LLMs fine-tuned on \dataset achieve assertion generation performance comparable to that of human experts. This is illustrated in the textbox \ref{tbox:hum_exp}. 
For instance, in example 1, when verifying whether the \texttt{bus\_release\_cnt} signal has been reset, the LLM-generated assertion takes the form \texttt{bus\_release\_cnt == '0'}, while the human expert expresses the same operation as \texttt{!(|bus\_release\_cnt)}. The latter format, often favored by experts, is typically chosen for its ease of writing and brevity. Similarly, in example 2, since \textit{mr\_err} is a one-bit flag, the human expert chooses to verify whether the flag was raised by writing \texttt{mr\_err} for the check, while the LLMs use the full expression, \texttt{mr\_err == 1'b1}.


% TO DO Explain 2 and 3

\input{Appendix_exmaples_Addressing_Issues/HumanExpert}
%\input{Tables/abl_table}





\subsection{Coverage Measurement}
\label{sec:coverage_measurement_appen}
Complete Path Coverage (CPC) refers to covering all possible independent paths within an automaton. A path begins at the initial node, traverses through the graph's edges, and ends at a final node. While CPC provides a thorough examination of the system, it becomes infeasible for graphs containing cycles, as these can result in infinite path lengths.

In our approach, we use complete path coverage as our primary coverage metric. This ensures a comprehensive evaluation of the system's behavior by accounting for all potential paths. To validate our coverage, we employed both formal and simulation-based verification tools, including \cite{jasper} and \cite{vivado}. These tools allowed us to rigorously analyze the generated assertions and ensure that they comprehensively cover all the functions defined within the system. By leveraging our method to extract properties from every possible conditional branch, we achieve up to 100\% coverage. This robust verification strategy confirms the correctness and reliability of the automaton's functionality across all defined behaviors.


% \subsection{Data Leakage Prevention}

% \textcolor{blue}{Experiments and writing in progress. In the GPT-3 paper (Language Models are Few-Shot Learners) the authors address data contamination by creating 'clean' versions of their benchmarks. They define potential contamination as examples that have a 13-gram overlap with any part of the pretraining set. This means that if a sequence of 13 consecutive tokens in the evaluation data appears in the training data, it is considered contaminated. The relevant section can be found in Appendix A.1 of the paper. In the PaLM paper (PaLM: Scaling Language Modeling with Pathways), the authors mention verifying that there was no data contamination between their model training corpus and the reasoning evaluation sets through n-gram overlap analysis.}




\subsection{Impact of Contamination on Assertion Generation}

Regarding potential data contamination, from our experiments, we observed that certain HDL components negatively impact the generation of syntactically and functionally correct assertions. Notably, module instantiations and ``\texttt{ifdef}'' commands challenge assertion generation. Specifically, the models used to evaluate VERT rarely generate assertions from module instantiations, leading to syntactically and functionally incorrect results. Moreover, these smaller models tend to misinterpret ``\texttt{ifdef}'' commands as conventional if-else statements. While this misclassification occurs infrequently, it reduces the percentage of correctly generated assertions. Assertions derived from these commands are often both syntactically incorrect—since ``\texttt{ifdef}'' commands do not adhere to standard if-else syntax and lack the necessary information for typical branching—and functionally incorrect, as they do not contribute meaningfully to functional branching. In contrast, GPT-4o appears unaffected by these HDL components in its assertion generation.
Table 1 illustrates the effect of increasing contamination in design files on assertion generation. Here, ``contamination'' refers to adding ``\texttt{ifdef}'' commands and module instantiations. For example, ``+10 contamination'' indicates that 10 additional instances of each of these elements (on top of the already existing instances) were introduced into the design files. The results show that as the level of contamination increases, the number of incorrectly generated assertions also rises. It should be noted that typically, in the hardware design, the number of ``\texttt{ifdef}'' commands is limited to at most five. Therefore, the scenarios used here to evaluate the contamination effect are unrealistic and to study the effect of contamination on the models.
\input{Tables/contamination}

Table \ref{tab:cont-table} illustrates the effect of increasing contamination in design files on assertion generation. Column 1, ``Models,'' specifies the LLM being tested, while Column 2, ``Benchmark/Hardware IP,'' lists the specific test benchmark used. Columns 3, 4, and 5, under ``Generated Assertions,'' indicate the total number of assertions generated with no contamination, an additional 10 contamination, and an additional 20 contamination in the input dataset, respectively. Columns 6, 7, and 8, under ``Syntactically Correct (\%),'' measure the percentage of assertions that are syntactically valid for each contamination level. Finally, Columns 9, 10, and 11, under ``Functionally Correct (\%),'' represent the percentage of assertions that are logically accurate and align with the intended functionality under the same contamination conditions. Here, ``contamination'' refers to the addition of ``\texttt{ifdef}'' commands and module instantiations. A contamination level lower than 10 was found to have a negligible impact on the results, while levels exceeding 20 were impractical due to exceeding the context size limitations of our models. The results show that as the level of contamination increases, the number of incorrectly generated assertions also rises. This results in a 3\% drop in accuracy.  It should be noted that typically, in the hardware design, the number of ``\texttt{ifdef}'' commands is limited to at most five. Therefore, the scenarios used here to evaluate the contamination effect are unrealistic and are used to study the effect of contamination on the models.



==> Snippets/listing_case.tex <==
\lstset{style=mystyle}
\begin{lstlisting}[language=Verilog]
...
case ( flag_register_18 )
   5'b10011 : begin
     chip_12 = tx_10;
   end
...
\end{lstlisting}

==> Snippets/listing_case_assertions.tex <==
\lstset{style=mystyle}
\begin{lstlisting}[language=Verilog]
...
property name;
( flag_register_18 ) == ( 5'b10011 ) 
|-> chip_12 == tx_10 ;
endproperty 
...
\end{lstlisting}

==> Snippets/listing_caseif.tex <==
\lstset{style=mystyle}
\begin{lstlisting}[language=Verilog]
...
case ( flag_register_18 ) 
    7'h26 : begin
...
    if (  rx_6  || rx_1  || hw_7 ) begin 
      cfg_20 = err_20;
      reg_3 = rst_15;
...
\end{lstlisting}

==> Snippets/listing_caseif_assertions.tex <==
\lstset{style=mystyle}
\begin{lstlisting}[language=Verilog]
...
property name;
( flag_register_18 ) == ( 7'h26 ) &&  
(  rx_6  || rx_1  || hw_7 ) |-> 
cfg_20 == err_20 && 
reg_3 == rst_15 ;
endproperty
...
\end{lstlisting}

==> Snippets/listing_ifelse.tex <==
\lstset{style=mystyle}
\begin{lstlisting}[language=Verilog]
...
if ( !cfg_7 ) begin 
...
 else if (  hw_13  && reg_14  || core_17 ) begin
  chip_9 = fsm_18;
...
\end{lstlisting}

==> Snippets/listing_ifelse_assertions.tex <==
\lstset{style=mystyle}
\begin{lstlisting}[language=Verilog]
...
property name; 
 (!cfg_7) && (hw_13 && reg_14 || core_17)
 |-> chip_9 == fsm_18;
endproperty
...


\end{lstlisting}

==> Tables/CVA6TABLE.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{}
\label{tab:cva6}
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Hardware IP/ Block & Module Name & Generated Assertions & Syntactically Correct Assertions & Functionally Correct Assertions & Missed Conditions & Wrong Condition \\ \hline
\multirow{33}{*}{CVA6} & acc\_dispatcher               & 9  &  &  &  &  \\ \cline{2-7} 
                       & alu                           & 7  &  &  &  &  \\ \cline{2-7} 
                       & ariane\_regfile               & 5  &  &  &  &  \\ \cline{2-7} 
                       & ariane\_regfile\_ff           & 5  &  &  &  &  \\ \cline{2-7} 
                       & ariane\_regfile\_fpga         & 6  &  &  &  &  \\ \cline{2-7} 
                       & axi\_shim                     & 4  &  &  &  &  \\ \cline{2-7} 
                       & commit\_stage                 & 3  &  &  &  &  \\ \cline{2-7} 
                       & compressed\_decoder           & 2  &  &  &  &  \\ \cline{2-7} 
                       & controller                    & 21 &  &  &  &  \\ \cline{2-7} 
                       & csr\_buffer                   & 6  &  &  &  &  \\ \cline{2-7} 
                       & csr\_regfile                  & 65 &  &  &  &  \\ \cline{2-7} 
                       & cva6                          & 1  &  &  &  &  \\ \cline{2-7} 
                       & cva6\_fifo\_v3                & 19 &  &  &  &  \\ \cline{2-7} 
                       & cva6\_rvfi                    & 17 &  &  &  &  \\ \cline{2-7} 
                       & cva6\_rvfi\_probes            & 2  &  &  &  &  \\ \cline{2-7} 
                       & cvxif\_compressed\_if\_driver & 6  &  &  &  &  \\ \cline{2-7} 
                       & cvxif\_fu                     & 2  &  &  &  &  \\ \cline{2-7} 
                       & decoder                       & 3  &  &  &  &  \\ \cline{2-7} 
                       & ex\_stage                     & 6  &  &  &  &  \\ \cline{2-7} 
                       & id\_stage                     & 2  &  &  &  &  \\ \cline{2-7} 
                       & instr\_realign                & 3  &  &  &  &  \\ \cline{2-7} 
                       & issue\_read\_operands         & 27 &  &  &  &  \\ \cline{2-7} 
                       & load\_store\_unit             & 4  &  &  &  &  \\ \cline{2-7} 
                       & load\_unit                    & 18 &  &  &  &  \\ \cline{2-7} 
                       & lsu\_bypass                   & 10 &  &  &  &  \\ \cline{2-7} 
                       & macro\_decoder                & 2  &  &  &  &  \\ \cline{2-7} 
                       & mult                          & 2  &  &  &  &  \\ \cline{2-7} 
                       & multiplier                    & 13 &  &  &  &  \\ \cline{2-7} 
                       & perf\_counters                & 4  &  &  &  &  \\ \cline{2-7} 
                       & scoreboard                    & 17 &  &  &  &  \\ \cline{2-7} 
                       & serdiv                        & 1  &  &  &  &  \\ \cline{2-7} 
                       & store\_buffer                 & 16 &  &  &  &  \\ \cline{2-7} 
                       & store\_unit                   & 4  &  &  &  &  \\ \hline
\end{tabular}%
}
\end{table}

==> Tables/DeepSeekRslt.tex <==
% \begin{table}[t]
% \centering
% \caption{Assertion Generation Results for the DeepSeek Model.}
% \label{tab:assert_rslt_deep}

% \resizebox{\columnwidth}{!}{%
% \renewcommand{\arraystretch}{1.2}
% \newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
% \begin{tabular}{|m{3.5cm}|M{3cm}|M{3cm}|M{3cm}|M{3cm}|}
% \hline
% \rowcolor[HTML]{c0c0c0}
% \textbf{Benchmark/Hardware IP} & \textbf{Generated Assertions} & \textbf{Syntactically Correct Assertions} & \textbf{Functionally Correct Assertions} & \textbf{Covered} \\ \hline \hline
% OpenTitan/AES        & 157 & 94.90       & 93.63       & 92.99 \\ \hline
% OpenTitan/I2C        & 124 & 97.58       & 97.58       & 97.58 \\ \hline
% OpenTitan/LC CTRL    & 19  & 100.00      & 100.00      & 100.00\\ \hline
% OpenTitan/ADC CTRL   & 32  & 100.00      & 96.88       & 96.88 \\ \hline
% %CVA6/Frontend        & 14  & 92.86       & 92.86       & 92.86 \\ \hline
% CVA6/Decode\&Issue   & 32  & 100.00      & 100.00      & 100.00\\ \hline
% CVA6/Execute         & 99  & 97.98       & 97.98       & 97.98 \\ \hline
% CVA6/Commit          & 93  & 89.25       & 89.25       & 89.25 \\ \hline
% CVA6/Controller\&Top & 76  & 89.47       & 89.47       & 89.47 \\ \hline
% \end{tabular}%

% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

% \usepackage{color}
% \usepackage{tabularray}



% \usepackage{color}
% \usepackage{tabularray}
\definecolor{Silver}{rgb}{0.752,0.752,0.752}
\begin{table}
\centering
\caption{Assertion Generation Results for the DeepSeek Model.}
\refstepcounter{table}
\label{tab:assert_rslt_deep}
\resizebox{\linewidth}{!}{%
\begin{tblr}{
  row{1} = {Silver,c},
  row{2} = {Silver,c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {c=2}{},
  cell{1}{4} = {c=2}{},
  cell{1}{6} = {c=2}{},
  cell{1}{8} = {c=2}{}, 
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{3}{7} = {c},
  cell{3}{8} = {c},
  cell{3}{9} = {c},
  cell{4}{2} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{4}{5} = {c},
  cell{4}{6} = {c},
  cell{4}{7} = {c},
  cell{4}{8} = {c},
  cell{4}{9} = {c},
  cell{5}{2} = {c},
  cell{5}{3} = {c},
  cell{5}{4} = {c},
  cell{5}{5} = {c},
  cell{5}{6} = {c},
  cell{5}{7} = {c},
  cell{5}{8} = {c},
  cell{5}{9} = {c},
  cell{6}{2} = {c},
  cell{6}{3} = {c},
  cell{6}{4} = {c},
  cell{6}{5} = {c},
  cell{6}{6} = {c},
  cell{6}{7} = {c},
  cell{6}{8} = {c},
  cell{6}{9} = {c},
  cell{7}{2} = {c},
  cell{7}{3} = {c},
  cell{7}{4} = {c},
  cell{7}{5} = {c},
  cell{7}{6} = {c},
  cell{7}{7} = {c},
  cell{7}{8} = {c},
  cell{7}{9} = {c},
  cell{8}{3} = {c},
  cell{8}{5} = {c},
  cell{8}{7} = {c},
  cell{8}{9} = {c},
  cell{9}{2} = {c},
  cell{9}{3} = {c},
  cell{9}{4} = {c},
  cell{9}{5} = {c},
  cell{9}{6} = {c},
  cell{9}{7} = {c},
  cell{9}{8} = {c},
  cell{9}{9} = {c},
  cell{10}{2} = {c},
  cell{10}{3} = {c},
  cell{10}{4} = {c},
  cell{10}{5} = {c},
  cell{10}{6} = {c},
  cell{10}{7} = {c},
  cell{10}{8} = {c},
  cell{10}{9} = {c},
  cell{11}{2} = {c},
  cell{11}{3} = {c},
  cell{11}{4} = {c},
  cell{11}{5} = {c},
  cell{11}{6} = {c},
  cell{11}{7} = {c},
  cell{11}{8} = {c},
  cell{11}{9} = {c},
  cell{12}{3} = {c},
  cell{12}{5} = {c},
  cell{12}{7} = {c},
  cell{12}{9} = {c},
  cell{13}{3} = {c},
  cell{13}{5} = {c},
  cell{13}{7} = {c},
  cell{13}{9} = {c},
  cell{14}{3} = {c},
  cell{14}{5} = {c},
  cell{14}{7} = {c},
  cell{14}{9} = {c},
  vlines,
  hline{1,4-15} = {-}{},
  hline{2} = {2-9}{},
  hline{3} = {-}{},
}
{\textbf{Benchmark/}\\\textbf{Hardware IP}}  & \textbf{Generated Assertions} &                                        & \textbf{Syntactically Correct Assertions, (\%)} &                                        & \textbf{Functionally Correct Assertions, (\%)} &                                        & \textbf{Assertion Coverage Rate, (\%)} &                                        \\
                             & \textbf{Base Model}           & {\textbf{Fine-Tuned}\\\textbf{ Model}} & \textbf{Base Model}                       & {\textbf{Fine-Tuned}\\\textbf{ Model}} & \textbf{Base Model}                      & {\textbf{Fine-Tuned}\\\textbf{ Model}} & \textbf{Base Model}              & {\textbf{Fine-Tuned}\\\textbf{ Model}} \\
OpenTitan/AES                & 148                              & 157                                 & 10.81                                          & 94.90                                  & 6.08                                   & 93.63                                  & 6.08                              & 92.99                                  \\
OpenTitan/I2C                & 132                              & 124                                    & 12.12                                          & 97.58                                  & 8.33                                         & 97.58                                  & 8.33                                 & 97.58                                  \\
OpenTitan/LC CTRL            & 21                              & 19                                     & 14.29                                          & 100.00                                 & 9.52                                         & 100.00                                 & 9.52                                 & 100.00                                 \\
OpenTitan/ADC CTRL           & 32                            & 32                                     & 6.25                                       & 100.00                                 & 0                                        & 96.88                                  & 0                                & 96.88                                  \\
CVA6/Frontend                & 16                              & 14                                     & 56.25                                          & 92.86                                  & 37.50                                         & 92.86                                  & 37.50                                 & 92.86                                  \\
CVA6/DecodeIssue             & 37                              & 32                                     & 18.92                                          & 100.00                                 & 13.51                                         & 100.00                                 & 13.51                                 & 100.00                                 \\
CVA6/Execute                 & 91                              & 99                                     & 26.37                                          & 97.98                                  & 20.88                                         & 97.98                                  & 20.88                                 & 97.98                                  \\
CVA6/Commit                  & 97                              & 93                                     & 21.65                                          & 89.25                                  & 17.53                                         & 89.25                                  & 17.53                                 & 89.25                                  \\
CVA6/ControllerTop           & 82                              & 76                                     & 21.95                                          & 89.47                                  & 15.85                                         & 89.47                                  & 15.85                                 & 89.47                                  \\
Pulpissimo/APB               &                               & 12                                     &                                           & 100.00                                 &                                          & 100.00                                 &                                  & 100.00                                 \\
Pulpissimo/RISCV/debug\_unit &                               & 19                                     &                                           & 100.00                                 &                                          & 100.00                                 &                                  & 100.00                                 \\
Pulpissimo/zero-riscy        &                               & 15                                     &                                           & 100.00                                 &                                          & 100.00                                 &                                  & 100.00                                 
\end{tblr}
}
\end{table}

==> Tables/LLama3Rslt.tex <==
\begin{table}[t]
\centering
\caption{Assertion Generation Results for the LLama3.1 Model.}
\label{tab:assert_rslt_llama}
\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.2}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{tabular}{|m{3.5cm}|M{3cm}|M{3cm}|M{3cm}|M{3cm}|}
\hline
\rowcolor[HTML]{c0c0c0} 
\textbf{Benchmark/Hardware IP} & \textbf{Generated Assertions} & \textbf{Syntactically Correct Assertions} & \textbf{Functionally Correct Assertions}   & \textbf{Covered} \\ \hline \hline
OpenTitan/AES        & 125 & 88.70           & 83.48           & 82.61 \\ \hline
OpenTitan/I2C        & 126 & 83.33           & 83.33           & 83.33 \\ \hline
OpenTitan/LC CTRL    & 19  & 89.47           & 89.47           & 89.47 \\ \hline
OpenTitan/ADC CTRL   & 32  & 100.00          & 100.00          & 100.00\\ \hline
CVA6/Frontend        & 13  & 92.31           & 92.31           & 92.31 \\ \hline
CVA6/Decode\&Issue   & 34  & 100.00          & 100.00          & 100.00\\ \hline
CVA6/Execute         & 105 & 91.43           & 91.43           & 91.43 \\ \hline
CVA6/Commit          & 79  & 89.87           & 89.87           & 89.87 \\ \hline
CVA6/Controller\&Top & 68  & 95.59           & 95.59           & 95.59 \\ \hline
\end{tabular}%
}
\end{table}


% m{3.5cm}M{3cm}M{3cm}M{3cm}M{3cm}

% \usepackage{color}
% \usepackage{tabularray}
\definecolor{Silver}{rgb}{0.752,0.752,0.752}
\begin{table}
\centering
\caption{Assertion Generation Results for the LLama3.1 Model.}
\refstepcounter{table}
\label{tab:assert_rslt_llama}
\resizebox{\linewidth}{!}{%
\begin{tblr}{
  row{1} = {Silver},
  row{2} = {Silver,c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {c=2}{c},
  cell{1}{4} = {c=2}{c},
  cell{1}{6} = {c=2}{c},
  cell{1}{8} = {c=2}{c},
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{3}{7} = {c},
  cell{3}{8} = {c},
  cell{3}{9} = {c},
  cell{4}{2} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{4}{5} = {c},
  cell{4}{6} = {c},
  cell{4}{7} = {c},
  cell{4}{8} = {c},
  cell{4}{9} = {c},
  cell{5}{2} = {c},
  cell{5}{3} = {c},
  cell{5}{4} = {c},
  cell{5}{5} = {c},
  cell{5}{6} = {c},
  cell{5}{7} = {c},
  cell{5}{8} = {c},
  cell{5}{9} = {c},
  cell{6}{2} = {c},
  cell{6}{3} = {c},
  cell{6}{4} = {c},
  cell{6}{5} = {c},
  cell{6}{6} = {c},
  cell{6}{7} = {c},
  cell{6}{8} = {c},
  cell{6}{9} = {c},
  cell{7}{2} = {c},
  cell{7}{3} = {c},
  cell{7}{4} = {c},
  cell{7}{5} = {c},
  cell{7}{6} = {c},
  cell{7}{7} = {c},
  cell{7}{8} = {c},
  cell{7}{9} = {c},
  cell{8}{2} = {c},
  cell{8}{3} = {c},
  cell{8}{4} = {c},
  cell{8}{5} = {c},
  cell{8}{6} = {c},
  cell{8}{7} = {c},
  cell{8}{8} = {c},
  cell{8}{9} = {c},
  cell{9}{2} = {c},
  cell{9}{3} = {c},
  cell{9}{4} = {c},
  cell{9}{5} = {c},
  cell{9}{6} = {c},
  cell{9}{7} = {c},
  cell{9}{8} = {c},
  cell{9}{9} = {c},
  cell{10}{2} = {c},
  cell{10}{3} = {c},
  cell{10}{4} = {c},
  cell{10}{5} = {c},
  cell{10}{6} = {c},
  cell{10}{7} = {c},
  cell{10}{8} = {c},
  cell{10}{9} = {c},
  cell{11}{2} = {c},
  cell{11}{3} = {c},
  cell{11}{4} = {c},
  cell{11}{5} = {c},
  cell{11}{6} = {c},
  cell{11}{7} = {c},
  cell{11}{8} = {c},
  cell{11}{9} = {c},
  cell{12}{2} = {c},
  cell{12}{3} = {c},
  cell{12}{4} = {c},
  cell{12}{5} = {c},
  cell{12}{6} = {c},
  cell{12}{7} = {c},
  cell{12}{8} = {c},
  cell{12}{9} = {c},
  cell{13}{2} = {c},
  cell{13}{3} = {c},
  cell{13}{4} = {c},
  cell{13}{5} = {c},
  cell{13}{6} = {c},
  cell{13}{7} = {c},
  cell{13}{8} = {c},
  cell{13}{9} = {c},
  cell{14}{2} = {c},
  cell{14}{3} = {c},
  cell{14}{4} = {c},
  cell{14}{5} = {c},
  cell{14}{6} = {c},
  cell{14}{7} = {c},
  cell{14}{8} = {c},
  cell{14}{9} = {c},
  vlines,
  hline{1,3-15} = {-}{},
  hline{2} = {2-9}{},
}
\textbf{Benchmark/Hardware IP} & \textbf{Generated Assertions} &                     & \textbf{Syntactically Correct Assertions, (\%)} &                     & \textbf{Functionally Correct Assertions, (\%)} &                     & \textbf{Assertion Coverage Rate, (\%)} &                     \\
                               & \textbf{Base Model}           & {\textbf{Fine-Tuned}\\\textbf{ Model}}  & \textbf{Base Model}                       & {\textbf{Fine-Tuned}\\\textbf{ Model}} & \textbf{Base Model}                      & {\textbf{Fine-Tuned}\\\textbf{ Model}} & \textbf{Base Model}              & {\textbf{Fine-Tuned}\\\textbf{ Model}} \\
OpenTitan/AES                  & 212                              & 125                 & 34.43                                          & 88.70               & 8.02                                         & 83.48               & 8.02                                 & 82.61               \\
OpenTitan/I2C                  &  149                             & 126                 &  28.19                                         & 83.33               & 8.72                                         & 83.33               & 8.72                                 & 83.33               \\
OpenTitan/LC CTRL              & 26                            & 19                  & 23.08                                       & 89.47              & 7.69                                      & 89.47               & 7.69                                 & 89.47               \\
OpenTitan/ADC CTRL             & 63                              & 32                  & 17.46                                        & 100.00              & 9.52                                         & 100.00              & 9.52                                 & 100.00              \\
CVA6/Frontend                  & 17                              & 13                  & 41.18                                          & 92.31               & 11.76                                         & 92.31               & 11.76                                 & 92.31               \\
CVA6/DecodeIssue               & 31                              & 34                  & 22.58                                          & 100.00              & 6.45                                         & 100.00              & 6.45                                 & 100.00              \\
CVA6/Execute                   & 110                              & 105                 & 24.55                                          & 91.43               & 5.45                                         & 91.43               & 5.45                                 & 91.43               \\
CVA6/Commit                    & 70                              & 79                  & 38.57
& 89.87               & 8.57                                         & 89.87               & 8.57                                 & 89.87               \\
CVA6/ControllerTop             & 73                              & 68                  & 32.88                                          & 95.59               & 5.48                                         & 95.59               & 5.48                                 & 95.59               \\
Pulpissimo/APB                 &  15                             & 19                  &       53.33                                    & 89.47               &      53.33                                    & 89.47               & 53.33                                 & 89.47               \\
Pulpissimo/RISCV/debug\_unit   & 19                              & 15                  &    21.05                                       & 93.33               &     21.05                                     & 93.33               & 21.05                                  & 93.33               \\
Pulpissimo/zero-riscy          &  6                             & 11                  &    16.67                                       & 100.00              &  16.67                                        & 100.00              &  16.67                                & 100.00              
\end{tblr}
}
\end{table}

% BASE MODEL REPETATIONS
% AES CIPER CONTROL - 4 ASSERTIONS from just the IF

==> Tables/Merged.tex <==
\begin{table}[t]
\centering
\caption{Assertion Generation Results for the DeepSeek Model.}
\label{tab:assert_rslt_deep}

\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.2}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{tabular}{|m{3.5cm}|M{3cm}|M{3cm}|M{3cm}|M{3cm}|}
\hline
\rowcolor[HTML]{c0c0c0}
\textbf{Benchmark/Hardware IP} & \textbf{Generated Assertions} & \textbf{Syntactically Correct Assertions} & \textbf{Functionally Correct Assertions} & \textbf{Covered} \\ \hline \hline
OpenTitan/AES      & 157 & 94.9  & 93.63 & 92.99 \\ \hline
OpenTitan/I2C      & 124 & 97.58 & 97.58 & 97.58 \\ \hline
OpenTitan/LC CTRL  & 19  & 100   & 100   & 100   \\ \hline
OpenTitan/ADC CTRL & 32  & 100   & 96.88 & 96.88 \\ \hline
CVA6               & 314 & 93.31 & 93.31 & 93.31 \\ \hline
\end{tabular}%

}
\end{table}

==> Tables/MistralRslt.tex <==
\begin{table}[t]
\centering
\caption{Assertion Generation Results for the Mistral Model.}
\label{tab:assert_rslt_mistral}
\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.2}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{tabular}{|m{3.5cm}|M{3cm}|M{3cm}|M{3cm}|M{3cm}|}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Benchmark/Hardware IP} & \textbf{Generated Assertions} & \textbf{Syntactically Correct Assertions} & \textbf{Functionally Correct Assertions} & \textbf{Covered} \\ \hline \hline
OpenTitan/AES      & 247 & 81.38    & 81.38    & 81.38    \\ \hline
OpenTitan/I2C      & 216 & 93.98    & 93.98    & 93.98    \\ \hline
OpenTitan/LC CTRL  & 10  & 80       & 80       & 80       \\ \hline
OpenTitan/ADC CTRL & 56  & 100      & 100      & 100      \\ \hline
CVA6               & 0   & \#DIV/0! & \#DIV/0! & \#DIV/0! \\ \hline
\end{tabular}%
}
\end{table}

==> Tables/OPENRISC.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Pulpisssimo}
\label{tab:pulp}
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Hardware IP/ Block & Module Name & Generated Assertions & Syntactically Correct Assertions & Functionally Correct Assertions & Missed Conditions & Wrong Condition \\ \hline
\multirow{17}{*}{Pulpissimo} & asic\_autogen\_rom                     & 1  &  &  &  &  \\ \cline{2-7} 
                             & cam\_vip                               & 8  &  &  &  &  \\ \cline{2-7} 
                             & fpga\_autogen\_rom                     & 1  &  &  &  &  \\ \cline{2-7} 
                             & fpga\_clk\_gen                         & 3  &  &  &  &  \\ \cline{2-7} 
                             & fpga\_slow\_clk\_gen                   & 4  &  &  &  &  \\ \cline{2-7} 
                             & gpio\_input\_stage                     & 2  &  &  &  &  \\ \cline{2-7} 
                             & gpio\_input\_stage\_no\_clk\_gates     & 2  &  &  &  &  \\ \cline{2-7} 
                             & jtag\_pkg                              & 54 &  &  &  &  \\ \cline{2-7} 
                             & pulpissimo\_padframe\_all\_pads\_muxer & 96 &  &  &  &  \\ \cline{2-7} 
                             & pulp\_clock\_gating\_xilinx            & 1  &  &  &  &  \\ \cline{2-7} 
                             & pulp\_tap\_pkg                         & 8  &  &  &  &  \\ \cline{2-7} 
                             & riscv\_pkg                             & 2  &  &  &  &  \\ \cline{2-7} 
                             & SimDTM                                 & 2  &  &  &  &  \\ \cline{2-7} 
                             & srec\_pkg                              & 5  &  &  &  &  \\ \cline{2-7} 
                             & tb\_gpio                               & 23 &  &  &  &  \\ \cline{2-7} 
                             & tb\_pulp                               & 8  &  &  &  &  \\ \cline{2-7} 
                             & tb\_pulp\_simple                       & 6  &  &  &  &  \\ \hline
\end{tabular}%
}
\end{table}

==> Tables/OPENTITANTABLE.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{}
\label{tab:OpenTitan}
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Hardware IP/ Block & Module Name & Generated Assertions & Syntactically Correct Assertions & Functionally Correct Assertions & Missed Conditions & Wrong Condition \\ \hline
\multirow{15}{*}{AES}     & cipher\_control\_fsm      & 9  & 8  & 7  & 1 & 0 \\ \cline{2-7} 
                          & cipher\_core              & 19 & 17 & 15 & 0 & 2 \\ \cline{2-7} 
                          & cipher\_control           & 6  & 6  & 5  & 0 & 1 \\ \cline{2-7} 
                          & key\_expand               & 3  & 3  & 3  & 0 & 0 \\ \cline{2-7} 
                          & ctr\_fsm                  & 5  & 4  & 3  & 0 & 1 \\ \cline{2-7} 
                          & Control\_fsm              & 9  & 9  & 8  & 0 & 1 \\ \cline{2-7} 
                          & core                      & 23 & 21 & 19 & 0 & 2 \\ \cline{2-7} 
                          & wrap                      & 8  & 7  & 4  & 1 & 2 \\ \cline{2-7} 
                          & ctrl\_reg\_shadowed       & 11 & 9  & 8  & 0 & 1 \\ \cline{2-7} 
                          & prng\_masking             & 6  & 4  & 0  & 4 & 0 \\ \cline{2-7} 
                          & aes                       & 2  & 2  & 2  & 0 & 0 \\ \cline{2-7} 
                          & Reg\_status               & 10 & 8  & 6  & 0 & 2 \\ \cline{2-7} 
                          & Reg\_top                  & 8  & 6  & 5  & 0 & 1 \\ \cline{2-7} 
                          & Sbox                      & 4  & 2  & 2  & 0 & 0 \\ \cline{2-7} 
                          & Sbox\_dom                 & 16 & 14 & 14 & 0 & 0 \\ \hline
\multirow{7}{*}{I2C}      & Bus\_monitor              & 23 & 21 & 18 & 3 & 0 \\ \cline{2-7} 
                          & Controller\_fsm           & 41 & 39 & 35 & 0 & 4 \\ \cline{2-7} 
                          & core                      & 5  & 4  & 4  & 0 & 1 \\ \cline{2-7} 
                          & fifo\_sync\_sram\_adapter & 8  & 6  & 5  & 0 & 1 \\ \cline{2-7} 
                          & fifos                     & 2  & 2  & 1  & 0 & 1 \\ \cline{2-7} 
                          & Reg\_top                  & 2  & 2  & 2  & 0 & 0 \\ \cline{2-7} 
                          & target\_fsm               & 41 & 39 & 34 & 1 & 4 \\ \hline
\multirow{4}{*}{LC CTRL}  & fsm                       & 10 & 8  & 7  & 1 & 0 \\ \cline{2-7} 
                          & Kmac\_if                  & 19 & 17 & 15 & 0 & 2 \\ \cline{2-7} 
                          & reg\_top                  & 5  & 3  & 2  & 0 & 1 \\ \cline{2-7} 
                          & lc\_ctrl                  & 3  & 2  & 2  & 0 & 0 \\ \hline
\multirow{3}{*}{ADC CTRL} & ctrl\_fsm                 & 21 & 20 & 16 & 3 & 1 \\ \cline{2-7} 
                          & Ctrl\_intr                & 10 & 8  & 7  & 0 & 1 \\ \cline{2-7} 
                          & cipher\_control           & 2  & 2  & 2  & 0 & 0 \\ \hline
\end{tabular}%
}
\end{table}
